SLADE: Detecting Dynamic Anomalies in Edge Streams without Labels via Self-Supervised Learning

To detect anomalies in real-world graphs, such as social, email, and financial networks, various approaches have been developed. While they typically assume static input graphs, most real-world graphs grow over time, naturally represented as edge streams. In this context, we aim to achieve three goals: (a) instantly detecting anomalies as they occur, (b) adapting to dynamically changing states, and (c) handling the scarcity of dynamic anomaly labels. In this paper, we propose SLADE (Self-supervised Learning for Anomaly Detection in Edge Streams) for rapid detection of dynamic anomalies in edge streams, without relying on labels. SLADE detects the shifts of nodes into abnormal states by observing deviations in their interaction patterns over time. To this end, it trains a deep neural network to perform two self-supervised tasks: (a) minimizing drift in node representations and (b) generating long-term interaction patterns from short-term ones. Failure in these tasks for a node signals its deviation from the norm. Notably, the neural network and tasks are carefully designed so that all required operations can be performed in constant time (w.r.t. the graph size) in response to each new edge in the input stream. In dynamic anomaly detection across four real-world datasets, SLADE outperforms nine competing methods, even those leveraging label supervision.

==> 05_analysis.tex <==
\section{Complexity Analysis}
\label{sec:analysis}

We analyze the time complexity of \method ``in action'' after being trained. Specifically, we examine the cost of (a) updating the memory in response to a newly arrived edge, and (b) calculating anomaly scores for a query node.

\smallsection{Memory Update}
Given a newly arriving edge, \method updates the memory vector of each endpoint using GRU. 
The total time complexity is dominated by that  of GRU, which is $\calO({d_{s}}^{2}+d_{s}d_{m})$~\citep{rotman2021shuffling}, where $d_{s}$ and $d_{m}$ indicate the dimensions of memory vectors and messages respectively.

\smallsection{Anomaly Scoring}
Give a query node, \method first aims to restore its memory vector using TGAT with input being a zero-masked memory of the query node and the memory vectors of its at most $k$ most recent neighbors.
Thus, the time complexity of obtaining reconstructed memory is $\calO(k{d_{s}}^{2})$~\citep{zheng2023temporal} if we assume, for simplicity, that the embedding dimension of the attention layers is the same as the dimension $d_{s}$ of the memory vectors.
Then, \method computes the similarities (a) between the updated memory and previous memory vectors and (b) between retained and restored memory vectors, taking $\mathcal{O}({d_{s}}^{2})$ time.
As a result, the overall time complexity of \method for anomaly scoring of a node is $\mathcal{O}(k{d_{s}}^{2})$.

\red{Here, \method has the $\mathcal{O}(k{d_{s}}^{2}+d_{s}d_{m})$ time complexity which is constant with respect to the graph's growth (number of nodes and edges) per memory update and anomaly scoring.}
%Here, since all hyperparameters ($k, d_{s}$, and $d_{m}$) are constant, \method has the constant (i.e., $\mathcal{O}(1)$) time complexity per memory update and anomaly scoring.
If we perform anomaly scoring (for each endpoint) only when each edge arrives,
the total complexity is linear in the number of  edges in the input CTDG so far.

==> abalation_study.tex <==

\begin{table}
    % \vspace{-1mm}
    \setlength{\tabcolsep}{5pt}
    \setlength\aboverulesep{0.5pt}
    \centering
    \small
    \scalebox{0.75}{
        \begin{tabular}{cccccccc}
            \toprule
            $\calL_{d}$ & $\calL_{r}$ & $sc_{d}$ & $sc_{r}$ & Wikipedia & Reddit & Bitcoin-alpha & Bitcoin-OTC \\
            \midrule
            \midrule
            \ding{51}   & -    & \ding{51}      & -         & 85.69 $\pm$ 1.17       & 48.89 $\pm$ 1.53      & \ul{76.38 $\pm$ 0.48}       & 73.87 $\pm$ 0.23       \\
            -           & \ding{51} & -     & \ding{51}    & \ul{87.57 $\pm$ 0.35}       & 61.77 $\pm$ 0.12      & 74.84 $\pm$ 0.40       & \bf{75.80 $\pm$ 0.26}          \\
            \ding{51}           & \ding{51}         & \ding{51} & - & 87.42 $\pm$ 1.06       & 48.51 $\pm$ 1.56       & \bf{76.45 $\pm$ 0.52}       & 74.10 $\pm$ 0.25         \\
            \ding{51}   & \ding{51} & -   & \ding{51}      & 84.64 $\pm$ 0.75  & \ul{71.33 $\pm$ 0.56}       & 75.24 $\pm$ 3.50       & 75.70 $\pm$ 0.21   \\
            \midrule
            \ding{51}   & \ding{51}  & \ding{51} & \ding{51} & \bf{87.75 $\pm$ 0.68}       & \bf{72.19 $\pm$ 0.60}       & 76.32 $\pm$ 0.28  & \bf{75.80 $\pm$ 0.19}       \\
            \bottomrule
        \end{tabular}
    }
    \normalsize
    \caption{Comparison of AUC (in \%) of \method and its variants that use a subset of the proposed components (i.e., memory drift loss $\calL_{d}$, memory reconstruction loss $\calL_{r}$, drift score $sc_{d}$, and reconstruction score $sc_{r}$).
    In most cases, \method with all components performs best, showing the effectiveness of each component.
   % In most cases, using a combination of different types of losses and scores leads to consistent and significant performance as they complement each other.
    }
    % \vspace{-2mm}
    \label{tab:comparison}
    % \vspace{-3mm}
\end{table}

==> accuracy.tex <==

% \begin{table*}[!t]
%     \setlength{\tabcolsep}{5pt}
%     \centering
%     \small
%     \scalebox{1}{
%         \begin{tabular}{clccccccccccc}
%             \toprule
%             & Method & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
%             \midrule
%             \midrule
%             \multirow{10}{*}{\rotatebox{90}{Supervised}} 
%                 & \MLP              & 60.32 $\pm$ 1.5   & 62.06 $\pm$ 2.3  & 76.27 $\pm$ 1.1        & 64.05 $\pm$ 1.4   & 81.18 $\pm$ 0.2   & 75.62 $\pm$ 9.5   & 79.19 $\pm$ 0.5       & 99.58 $\pm$ 0.3   & 65.17 $\pm$ 2.3   & 93.75 $\pm$ 0.6  & 12.5   \\
%                 & \GCN\!$^{\star}$  & 77.11 $\pm$ 1.8   & 66.07 $\pm$ 2.4  & 82.63 $\pm$ 0.6        & 73.66 $\pm$ 1.3   & 87.58 $\pm$ 0.2   & 36.79 $\pm$ 9.6   & OOM                   & 92.47 $\pm$ 0.9   & 71.17 $\pm$ 2.4   & 91.67 $\pm$ 0.2  & 11.7   \\
%                 & \GAT\!$^{\star}$  & 77.75 $\pm$ 2.1   & 67.62 $\pm$ 2.5  & 81.96 $\pm$ 0.7        & 74.52 $\pm$ 1.3   & 88.59 $\pm$ 0.1   & 36.48 $\pm$ 10.0  & OOM                   & OOM               & 70.94 $\pm$ 2.6   & 91.43 $\pm$ 0.3  & 11     \\
%                 & \HGNN             & 77.50 $\pm$ 1.8   & 66.16 $\pm$ 2.3  & 83.52 $\pm$ 0.7        & 74.38 $\pm$ 1.2   & 88.32 $\pm$ 0.3   & 78.58 $\pm$ 11.1  & 80.15 $\pm$ 0.3       & 98.59 $\pm$ 0.5   & 72.03 $\pm$ 2.4   & 92.23 $\pm$ 0.2  & 8.1    \\
%                 & \HyperConv        & 76.19 $\pm$ 2.1   & 64.12 $\pm$ 2.6  & 83.42 $\pm$ 0.6        & 73.52 $\pm$ 1.0   & 88.83 $\pm$ 0.2   & 62.53 $\pm$ 14.5  & 79.83 $\pm$ 0.4       & 97.56 $\pm$ 0.6   & 72.62 $\pm$ 2.6   & 91.84 $\pm$ 0.1  & 9.8    \\
%                 & \HNHN             & 76.21 $\pm$ 1.7   & 67.28 $\pm$ 2.2  & 80.97 $\pm$ 0.9        & 74.88 $\pm$ 1.6   & 86.71 $\pm$ 1.2   & 78.89 $\pm$ 10.2  & 79.51 $\pm$ 0.4       & 99.78 $\pm$ 0.1   & 71.45 $\pm$ 3.2   & 92.96 $\pm$ 0.2  & 8.9    \\
%                 & \HyperGCN         & 64.11 $\pm$ 7.4   & 59.92 $\pm$ 9.6  & 78.40 $\pm$ 9.2        & 60.65 $\pm$ 9.2   & 76.59 $\pm$ 7.6   & 40.86 $\pm$ 2.1   & 77.31 $\pm$ 6.0       & 48.26 $\pm$ 0.3   & 46.05 $\pm$ 3.9   & 69.23 $\pm$ 2.8  & 15.1   \\
%                 & \HyperSAGE        & 64.98 $\pm$ 5.3   & 52.43 $\pm$ 9.4  & 79.49 $\pm$ 8.7        & 64.59 $\pm$ 4.3   & 79.63 $\pm$ 8.6   & 40.86 $\pm$ 2.1   & OOT              & OOT          & OOT          & OOT         & 14.7   \\
%                 & \UniGCN           & 77.91 $\pm$ 1.9   & 66.40 $\pm$ 1.9  & \ul{84.08 $\pm$ 0.7}   & 77.30 $\pm$ 1.4   & 90.31 $\pm$ 0.2   & 72.10 $\pm$ 12.1  & \tb{80.24 $\pm$ 0.4}  & 98.84 $\pm$ 0.5   & 73.27 $\pm$ 2.7   & 94.62 $\pm$ 0.2  & 5.9    \\
%                 & \AllSet           & 76.21 $\pm$ 1.7   & 67.83 $\pm$ 1.8  & 82.85 $\pm$ 0.9        & 76.94 $\pm$ 1.3   & 90.07 $\pm$ 0.3   & 72.72 $\pm$ 11.8  & 79.90 $\pm$ 0.4       & 99.78 $\pm$ 0.1   & 75.09 $\pm$ 2.5   & 96.85 $\pm$ 0.2  & 6.2    \\
%             \midrule
%             \multirow{8}{*}{\rotatebox{90}{Unsupervised}}
%                 & \Nodetovec\!$^{\star}$    & 70.99 $\pm$ 1.4   & 53.85 $\pm$ 1.9   & 78.75 $\pm$ 0.9   & 58.50 $\pm$ 2.1   & 72.09 $\pm$ 0.3   & 17.02 $\pm$ 4.1   & 63.35 $\pm$ 1.7   & 88.16 $\pm$ 0.8   & 67.72 $\pm$ 2.1   & 84.94 $\pm$ 0.4   & 15.6  \\
%                 & \DGI\!$^{\star}$          & 78.17 $\pm$ 1.4   & 68.81 $\pm$ 1.8   & 80.83 $\pm$ 0.6   & 76.94 $\pm$ 1.1   & 88.00 $\pm$ 0.2   & 36.54 $\pm$ 9.7   & OOM               & OOM               & 72.01 $\pm$ 2.5   & 92.18 $\pm$ 0.2   & 9.3   \\
%                 & \GRACE\!$^{\star}$        & 79.11 $\pm$ 1.7   & 68.65 $\pm$ 1.7   & 80.08 $\pm$ 0.7   & 76.59 $\pm$ 1.0   & OOM               & 37.07 $\pm$ 9.3   & OOM               & OOM               & 70.51 $\pm$ 2.4   & 90.68 $\pm$ 0.3   & 10.4  \\
%                 & \HHGR                     & 78.08 $\pm$ 1.7   & 68.21 $\pm$ 1.8   & 82.13 $\pm$ 0.6   & 78.15 $\pm$ 1.1   & 88.69 $\pm$ 0.2   & 80.06 $\pm$ 11.1  & 79.75 $\pm$ 0.3   & 97.15 $\pm$ 0.5   & 73.95 $\pm$ 2.4   & 93.26 $\pm$ 0.2   & 6.8   \\
%                 \cmidrule{2-13}
%                 & \RandomInit           & 63.62 $\pm$ 3.1       & 60.44 $\pm$ 2.5       & 67.49 $\pm$ 2.2       & 66.27 $\pm$ 2.2       & 76.57 $\pm$ 0.6       & 78.43 $\pm$ 11.0      & 77.14 $\pm$ 0.6       & 97.40 $\pm$ 0.6       & 74.39 $\pm$ 2.6       & 96.29 $\pm$ 0.3       & 11.9      \\
%                 & \tb{\methodN}         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5       & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 79.94 $\pm$ 11.1      & \ul{80.18 $\pm$ 0.2}  & 99.76 $\pm$ 0.2       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 3.4       \\
%                 & \tb{\methodNE}        & \ul{81.45 $\pm$ 1.2}  & \ul{71.38 $\pm$ 1.2}  & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & \ul{80.19 $\pm$ 11.1} & \ul{80.18 $\pm$ 0.2}  & \ul{99.81 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & \ul{97.02 $\pm$ 0.1}  & \ul{2}    \\
%                 & \tb{\method}          & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.2}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \tb{80.25 $\pm$ 11.2} & 80.14 $\pm$ 0.2       & \tb{99.83 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.5}  \\
%             \bottomrule
%         \end{tabular}
%     }
%     \normalsize
%     \vspace{-2mm}
%     \caption{Node classification accuracy and standard deviations. 
%     Graph methods, marked as $\star$, are applied after converting hypergraphs to graphs via clique expansion.
%     For each dataset, the best and the second-best performances are highlighted in boldface and underlined, respectively.
%     A.R. denotes average rank, OOT denotes cases where results are not obtained within 24 hours, and OOM indicates out of memory on a 24GB GPU.
%     In most cases, \method outperforms all others, including the supervised ones.
%     }
%     \label{tab:accuracy}
% \end{table*}





\begin{table*}[!t]
    \setlength{\tabcolsep}{5pt}
    \setlength\aboverulesep{0.5pt}
    \centering
    \small
    \scalebox{1}{
        \begin{tabular}{clcccccccc}
            \toprule
            & Method & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            \midrule
            \midrule
            \multirow{10}{*}{\rotatebox{90}{Supervised}} 
                & \MLP              & 60.32 $\pm$ 1.5   & 62.06 $\pm$ 2.3  & 76.27 $\pm$ 1.1        & 64.05 $\pm$ 1.4   & 81.18 $\pm$ 0.2   & 65.17 $\pm$ 2.3   & 93.75 $\pm$ 0.6   & 14.4   \\
                & \GCN\!$^{\star}$  & 77.11 $\pm$ 1.8   & 66.07 $\pm$ 2.4  & 82.63 $\pm$ 0.6        & 73.66 $\pm$ 1.3   & 87.58 $\pm$ 0.2   & 71.17 $\pm$ 2.4   & 91.67 $\pm$ 0.2   & 11.1   \\
                & \GAT\!$^{\star}$  & 77.75 $\pm$ 2.1   & 67.62 $\pm$ 2.5  & 81.96 $\pm$ 0.7        & 74.52 $\pm$ 1.3   & 88.59 $\pm$ 0.1   & 70.94 $\pm$ 2.6   & 91.43 $\pm$ 0.3   & 10.1     \\
                & \HGNN             & 77.50 $\pm$ 1.8   & 66.16 $\pm$ 2.3  & 83.52 $\pm$ 0.7        & 74.38 $\pm$ 1.2   & 88.32 $\pm$ 0.3   & 72.03 $\pm$ 2.4   & 92.23 $\pm$ 0.2   & 9    \\
                & \HyperConv        & 76.19 $\pm$ 2.1   & 64.12 $\pm$ 2.6  & 83.42 $\pm$ 0.6        & 73.52 $\pm$ 1.0   & 88.83 $\pm$ 0.2   & 72.62 $\pm$ 2.6   & 91.84 $\pm$ 0.1   & 10.1    \\
                & \HNHN             & 76.21 $\pm$ 1.7   & 67.28 $\pm$ 2.2  & 80.97 $\pm$ 0.9        & 74.88 $\pm$ 1.6   & 86.71 $\pm$ 1.2   & 71.45 $\pm$ 3.2   & 92.96 $\pm$ 0.2   & 10.3    \\
                & \HyperGCN         & 64.11 $\pm$ 7.4   & 59.92 $\pm$ 9.6  & 78.40 $\pm$ 9.2        & 60.65 $\pm$ 9.2   & 76.59 $\pm$ 7.6   & 46.05 $\pm$ 3.9   & 69.23 $\pm$ 2.8   & 16.3   \\
                & \HyperSAGE        & 64.98 $\pm$ 5.3   & 52.43 $\pm$ 9.4  & 79.49 $\pm$ 8.7        & 64.59 $\pm$ 4.3   & 79.63 $\pm$ 8.6   & OOT               & OOT               & 16   \\
                & \UniGCN           & 77.91 $\pm$ 1.9   & 66.40 $\pm$ 1.9  & \ul{84.08 $\pm$ 0.7}   & 77.30 $\pm$ 1.4   & 90.31 $\pm$ 0.2   & 73.27 $\pm$ 2.7   & 94.62 $\pm$ 0.2   & 5.9    \\
                & \AllSet           & 76.21 $\pm$ 1.7   & 67.83 $\pm$ 1.8  & 82.85 $\pm$ 0.9        & 76.94 $\pm$ 1.3   & 90.07 $\pm$ 0.3   & 75.09 $\pm$ 2.5   & 96.85 $\pm$ 0.2   & 6.3    \\
            \midrule
            \multirow{8}{*}{\rotatebox{90}{Unsupervised}}
                & \Nodetovec\!$^{\star}$    & 70.99 $\pm$ 1.4   & 53.85 $\pm$ 1.9   & 78.75 $\pm$ 0.9   & 58.50 $\pm$ 2.1   & 72.09 $\pm$ 0.3   & 67.72 $\pm$ 2.1   & 84.94 $\pm$ 0.4   & 16  \\
                & \DGI\!$^{\star}$          & 78.17 $\pm$ 1.4   & 68.81 $\pm$ 1.8   & 80.83 $\pm$ 0.6   & 76.94 $\pm$ 1.1   & 88.00 $\pm$ 0.2   & 72.01 $\pm$ 2.5   & 92.18 $\pm$ 0.2   & 8.3   \\
                & \GRACE\!$^{\star}$        & 79.11 $\pm$ 1.7   & 68.65 $\pm$ 1.7   & 80.08 $\pm$ 0.7   & 76.59 $\pm$ 1.0   & OOM               & 70.51 $\pm$ 2.4   & 90.68 $\pm$ 0.3   & 11  \\
                & \HHGR                     & 78.08 $\pm$ 1.7   & 68.21 $\pm$ 1.8   & 82.13 $\pm$ 0.6   & 78.15 $\pm$ 1.1   & 88.69 $\pm$ 0.2   & 73.95 $\pm$ 2.4   & 93.26 $\pm$ 0.2   & 6.6   \\
                \cmidrule{2-10}
                & \RandomInit           & 63.62 $\pm$ 3.1       & 60.44 $\pm$ 2.5       & 67.49 $\pm$ 2.2       & 66.27 $\pm$ 2.2       & 76.57 $\pm$ 0.6       & 74.39 $\pm$ 2.6       & 96.29 $\pm$ 0.3       & 12.9      \\
                & \tb{\methodN}         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5       & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 3.3       \\
                & \tb{\methodNE}        & \ul{81.45 $\pm$ 1.2}  & \ul{71.38 $\pm$ 1.2}  & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & \ul{97.02 $\pm$ 0.1}  & \ul{2}    \\
                & \tb{\method}          & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.2}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.1}  \\
            \bottomrule
        \end{tabular}
    }
    \normalsize
    % \vspace{-2mm}
    \caption{Node classification accuracy and standard deviations. 
    Graph methods, marked as $\star$, are applied after converting hypergraphs to graphs via clique expansion.
    For each dataset, the best and the second-best performances are highlighted in boldface and underlined, respectively.
    A.R. denotes average rank, OOT denotes cases where results are not obtained within 24 hours, and OOM indicates out of memory on a 24GB GPU.
    In most cases, \method outperforms all others, including the supervised ones.
    }
    \label{tab:accuracy}
\end{table*}

==> accuracy2.tex <==
\begin{table*}
    % \vspace{-2mm}
    \caption{Node classification accuracy in percentage along with standard deviations. 
    Graph algorithms, marked as $\star$, are applied after converting hypergraphs to graphs via clique expansion.
    For each dataset, the highest and the second-highest performance is highlighted in \textbf{boldface} and \underline{underlined}, respectively.
    A.R. denotes average rank, Time-out represents cases where results are not obtained within 24 hours, and OOM indicates out of memory on a 24GB GPU. 
    % Note that only the listed datasets are used to compute average rank.
    }
    \label{tab:accuracy2}
    \centering
    \scalebox{0.8}{
        \begin{tabular}{clcccccc}
            \toprule
            % \multirow{2}{*}{} & \multirow{2}{*}[-1mm]{Method} & \multicolumn{3}{c}{Co-citation Data} & \multicolumn{2}{c}{Co-authorship Data} & \multirow{2}{*}[-1mm]{A.R.$\downarrow$} \\
            & Method & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            % \cmidrule(lr){3-5} \cmidrule(lr){6-7}
            % & & Cora & Citeseer & Pubmed & Cora & DBLP \\
            \midrule
            \midrule
            \multirow{10}{*}{\rotatebox{90}{Supervised}} 
                & \MLP              & 75.62 $\pm$ 9.47  & 79.19 $\pm$ 0.45  & 99.58 $\pm$ 0.29  & 65.17 $\pm$ 2.32  & 93.75 $\pm$ 0.61  & 8.8   \\
                & \GCN\!$^{\star}$  & 36.79 $\pm$ 9.59  & OOM               & 92.47 $\pm$ 0.89  & 71.17 $\pm$ 2.36  & 91.67 $\pm$ 0.21  & 13    \\
                & \GAT\!$^{\star}$  & 36.48 $\pm$ 10.0  & OOM               & OOM               & 70.94 $\pm$ 2.55  & 91.43 $\pm$ 0.26  & 14.7  \\
                & \HGNN             & 78.58 $\pm$ 11.1  & 80.15 $\pm$ 0.25  & 98.59 $\pm$ 0.48  & 72.03 $\pm$ 2.41  & 92.23 $\pm$ 0.16  & 7     \\
                & \HyperConv        & 62.53 $\pm$ 14.5  & 79.83 $\pm$ 0.36  & 97.56 $\pm$ 0.64  & 72.62 $\pm$ 2.64  & 91.84 $\pm$ 0.14  & 9.4   \\
                & \HNHN             & 78.89 $\pm$ 10.2  & 79.51 $\pm$ 0.43  & \textbf{99.78 $\pm$ 0.10}  & 71.45 $\pm$ 3.16  & 92.96 $\pm$ 0.17  & 7     \\
                & \HyperGCN         & 40.86 $\pm$ 2.10  & 77.31 $\pm$ 6.04  & 48.26 $\pm$ 0.26  & 46.05 $\pm$ 3.91  & 69.23 $\pm$ 2.83  & 14.2  \\
                & \HyperSAGE        & 40.86 $\pm$ 2.10  & Time-out          & Time-out          & Time-out          & Time-out          & -     \\
                & \UniGCN           & 72.10 $\pm$ 12.1  & \textbf{80.24 $\pm$ 0.36}  & 98.84 $\pm$ 0.53  & 73.27 $\pm$ 2.69  & 94.62 $\pm$ 0.19  & 6.2   \\
                & \AllSet           & 72.72 $\pm$ 11.8  & 79.90 $\pm$ 0.43  & \underline{99.78 $\pm$ 0.13}  & 75.09 $\pm$ 2.50  & 96.85 $\pm$ 0.21  & 4.8   \\
            \midrule
            \multirow{8}{*}{\rotatebox{90}{Unsupervised}}
                & \Nodetovec\!$^{\star}$  & 17.02 $\pm$ 4.12  & 63.35 $\pm$ 1.74    & 88.16 $\pm$ 0.77  & 67.72 $\pm$ 2.13  & 84.94 $\pm$ 0.44  & 15    \\
                & \DGI\!$^{\star}$        & 36.54 $\pm$ 9.67  & OOM                 & OOM               & 72.01 $\pm$ 2.51  & 92.18 $\pm$ 0.20  & 12.3  \\
                & \GRACE\!$^{\star}$      & 37.07 $\pm$ 9.30  & OOM                 & OOM               & 70.51 $\pm$ 2.38  & 90.68 $\pm$ 0.25  & 14.3  \\
                & \HHGR                 & \underline{80.06 $\pm$ 11.1}  & 79.75 $\pm$ 0.32      & 97.15 $\pm$ 0.49  & 73.95 $\pm$ 2.44  & 93.26 $\pm$ 0.18  & 7.2   \\
                \cmidrule{2-8}
                & \RandomInit           & 78.43 $\pm$ 11.0  & 77.14 $\pm$ 0.58  & 97.40 $\pm$ 0.58  & 74.39 $\pm$ 2.57  & 96.29 $\pm$ 0.28  & 7.8   \\
                & \textbf{\methodN}     & 79.77 $\pm$ 10.9  & 80.14 $\pm$ 0.23  & 99.54 $\pm$ 0.23  & 75.11 $\pm$ 2.52  & 97.01 $\pm$ 0.15  & 4.2   \\
                & \textbf{\methodNE}    & 79.99 $\pm$ 10.9  & 80.17 $\pm$ 0.22  & 99.65 $\pm$ 0.19  & \underline{75.14 $\pm$ 2.51}  & \underline{97.02 $\pm$ 0.14}  & \underline{2.6}   \\
                & \textbf{\method}      & \textbf{80.11 $\pm$ 11.1}  & 80.12 $\pm$ 0.20  & 99.67 $\pm$ 0.19  & \textbf{75.17 $\pm$ 2.49}  & \textbf{97.08 $\pm$ 0.13}  & \textbf{2.2}   \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

==> backbone.tex <==
\begin{table}[!t]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lcc}
            \toprule
            Dataset & \method (with \HGNN) & \method (Proposed) \\
            \midrule
            \midrule
            Cora-C      & 81.03 $\pm$ 1.31  & \textbf{81.57 $\pm$ 1.12} \\
            Citeseer    & 71.97 $\pm$ 1.26  & \textbf{72.02 $\pm$ 1.16} \\
            Pubmed      & 83.80 $\pm$ 0.63  & \textbf{84.26 $\pm$ 0.62} \\
            Cora-A      & \textbf{82.22 $\pm$ 1.09}  & 82.15 $\pm$ 0.89 \\
            DBLP        & 90.93 $\pm$ 0.16  & \textbf{91.12 $\pm$ 0.11} \\
            Zoo         & 79.47 $\pm$ 11.0  & \textbf{80.25 $\pm$ 11.2} \\
            20News      & 79.93 $\pm$ 0.24  & \textbf{80.14 $\pm$ 0.19} \\
            Mushroom    & 98.93 $\pm$ 0.33  & \textbf{99.83 $\pm$ 0.13} \\
            NTU2012     & 74.63 $\pm$ 2.53  & \textbf{75.23 $\pm$ 2.45} \\
            ModelNet40  & \textbf{97.33 $\pm$ 0.14}  & 97.08 $\pm$ 0.13 \\
            \bottomrule
        \end{tabular}
    }
    \caption{
    The accuracy of two \method methods that use (1) \HGNN and (2) the mean pooling layer (proposed), respectively, as an encoder. 
    % \method using the mean pooling layer consistently and slightly outperforms the one using \HGNN as an encoder. 
    % This result justifies our choice of using the mean pooling layer as our backbone encoder.
    }
    \label{tab:backbone}
    \vspace{-2mm}
\end{table}

==> comparison.tex <==



% \begin{table*}
%     \vspace{-1mm}
%     \setlength{\tabcolsep}{5pt}
%     \centering
%     \small
%     \scalebox{1}{
%         \begin{tabular}{cccccccccccccc}
%             \toprule
%             $\calL_{n}$ & $\calL_{g}$ & $\calL_{m}$ & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
%             \midrule
%             \midrule
%             \ding{51}   & -         & -         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5*      & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 79.94 $\pm$ 11.1      & \tb{80.18 $\pm$ 0.2}  & 99.76 $\pm$ 0.2       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 3.8       \\
%             -           & \ding{51} & -         & 79.69 $\pm$ 1.6       & 71.02 $\pm$ 1.3*      & 80.20 $\pm$ 1.3       & 78.98 $\pm$ 1.4       & 88.60 $\pm$ 0.2       & 79.31 $\pm$ 10.7      & 79.35 $\pm$ 0.4       & 99.13 $\pm$ 0.3       & 74.41 $\pm$ 2.6       & 96.66 $\pm$ 0.2       & 5.7       \\
%             -           & -         & \ding{51} & 76.76 $\pm$ 1.8       & 63.98 $\pm$ 2.0       & 79.86 $\pm$ 0.9       & 76.77 $\pm$ 1.1       & 63.95 $\pm$ 7.2       & 79.80 $\pm$ 11.0      & 79.27 $\pm$ 0.3       & 94.87 $\pm$ 0.7       & 73.11 $\pm$ 2.8       & 96.57 $\pm$ 0.2       & 6.9       \\
%             \ding{51}   & \ding{51} & -         & \ul{81.45 $\pm$ 1.2}  & 71.38 $\pm$ 1.4       & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & 80.19 $\pm$ 11.1      & \tb{80.18 $\pm$ 0.2}  & \ul{99.81 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & 97.02 $\pm$ 0.1       & \ul{2.3}  \\
%             \ding{51}   & -         & \ding{51} & 80.49 $\pm$ 1.3       & 70.46 $\pm$ 1.5       & \ul{83.98 $\pm$ 0.7}  & 81.62 $\pm$ 1.0       & 90.75 $\pm$ 0.1       & 80.19 $\pm$ 11.1      & 80.15 $\pm$ 0.2       & 99.74 $\pm$ 0.2       & 75.12 $\pm$ 2.5       & \ul{97.03 $\pm$ 0.1}  & 3.6       \\
%             -           & \ding{51} & \ding{51} & 80.80 $\pm$ 1.1       & \ul{71.73 $\pm$ 1.4}  & 82.81 $\pm$ 0.7       & 80.24 $\pm$ 1.0       & 90.17 $\pm$ 0.1       & \ul{80.20 $\pm$ 11.1} & 79.29 $\pm$ 0.2       & 99.82 $\pm$ 0.1       & 73.76 $\pm$ 2.5       & 96.74 $\pm$ 0.1       & 4.1       \\
%             \ding{51}   & \ding{51} & \ding{51} & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.4}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \tb{80.25 $\pm$ 11.2} & 80.14 $\pm$ 0.2       & \tb{99.83 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.4}  \\
%             \bottomrule
%         \end{tabular}
%     }
%     \normalsize
%     \vspace{-2mm}
%     \caption{Comparison of node classification accuracy according to whether or not to use each type of contrast (i.e., $\calL_{n}$, $\calL_{g}$, and $\calL_{m}$). %(i.e., node, hyperedge, and membership-level contrast) 
%     Using all types of contrasts (i.e., node-, group-, and membership-level contrast) achieves the best performance in most cases as they are complementarily reinforcing each other.
%     }
%     \label{tab:comparison}
%     \vspace{-3mm}
% \end{table*}


\begin{table*}
    % \vspace{-1mm}
    \setlength{\tabcolsep}{5pt}
    \setlength\aboverulesep{0.5pt}
    \centering
    \small
    \scalebox{1}{
        \begin{tabular}{ccccccccccc}
            \toprule
            $\calL_{n}$ & $\calL_{g}$ & $\calL_{m}$ & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            \midrule
            \midrule
            \ding{51}   & -         & -         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5*      & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 4      \\
            -           & \ding{51} & -         & 79.69 $\pm$ 1.6       & 71.02 $\pm$ 1.3*      & 80.20 $\pm$ 1.3       & 78.98 $\pm$ 1.4       & 88.60 $\pm$ 0.2       & 74.41 $\pm$ 2.6       & 96.66 $\pm$ 0.2       & 5.6       \\
            -           & -         & \ding{51} & 76.76 $\pm$ 1.8       & 63.98 $\pm$ 2.0       & 79.86 $\pm$ 0.9       & 76.77 $\pm$ 1.1       & 63.95 $\pm$ 7.2       & 73.11 $\pm$ 2.8       & 96.57 $\pm$ 0.2       & 7       \\
            \ding{51}   & \ding{51} & -         & \ul{81.45 $\pm$ 1.2}  & 71.38 $\pm$ 1.4       & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & 97.02 $\pm$ 0.1       & \ul{2.3}  \\
            \ding{51}   & -         & \ding{51} & 80.49 $\pm$ 1.3       & 70.46 $\pm$ 1.5       & \ul{83.98 $\pm$ 0.7}  & 81.62 $\pm$ 1.0       & 90.75 $\pm$ 0.1       & 75.12 $\pm$ 2.5       & \ul{97.03 $\pm$ 0.1}  & 3.6       \\
            -           & \ding{51} & \ding{51} & 80.80 $\pm$ 1.1       & \ul{71.73 $\pm$ 1.4}  & 82.81 $\pm$ 0.7       & 80.24 $\pm$ 1.0       & 90.17 $\pm$ 0.1       & 73.76 $\pm$ 2.5       & 96.74 $\pm$ 0.1       & 4.4       \\
            \ding{51}   & \ding{51} & \ding{51} & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.4}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.1}  \\
            \bottomrule
        \end{tabular}
    }
    \normalsize
    % \vspace{-2mm}
    \caption{Comparison of node classification accuracy according to whether or not to use each type of contrast (i.e., $\calL_{n}$, $\calL_{g}$, and $\calL_{m}$). %(i.e., node, hyperedge, and membership-level contrast) 
    Using all types of contrasts (i.e., node-, group-, and membership-level contrast) achieves the best performance in most cases as they are complementarily reinforcing each other.
    }
    \label{tab:comparison}
    % \vspace{-3mm}
\end{table*}

==> dataset.tex <==
\begin{table}[!t]
    \centering
    \scalebox{0.75}{
        \begin{tabular}{lcccc}
            \toprule
             & Wikipedia & Reddit & Bitcoin-alpha & Bitcoin-OTC \\
            \midrule
                \# Nodes             & 9,227  & 10,984     & 3,783     & 5,881  \\
                \# Edges        & 157,474  & 672,447     & 24,186     & 35,592   \\
                \# Features       & 172  & 172     & 0    & 0 \\
                \# anomalies    & 217   & 366      & 1520      & 4344        \\
                anomalies ratio    & 0.14\%   & 0.05\%      & 6.28\%      & 12.20\%        \\   
                anomaly type    & post ban   & edit ban      & Unreliable user      & Unreliable user        \\
            \bottomrule
        \end{tabular}
    }
    \caption{Statistics of datasets used in our experiments. The count of anomalies refers to the number of edges where the dynamic state of the actor node is abnormal, and the ratio represents the proportion of these abnormal edges in relation to the total number of edges.}
    \label{tab:dataset}
\end{table}

==> main_alg.tex <==
% \begin{figure}[t]
% \vspace{-2mm}
\begin{algorithm}[t]
\small
\caption{\generator: Transitive hypergraph generator\label{algo:generator}}
\KwIn{(1) Number of nodes $n$, hyperedge size distribution $S$ \newline 
(2) Community size $C$, intra-community hyperedge ratio $p$ \newline
(3) Level-sampling coefficient $\alpha$, level-size coefficient $\beta$}
\KwOut{Generated hypergraph $G' = (V', E')$}

% \state Initialize node index $idx=1$, level index $T = 1$, hash table $\Psi_{L}$, hyperedge set $E' = \emptyset$, and number of hyperedges $m = S.$size() \\ 
$idx \leftarrow 1$; $T \leftarrow 0$; $\Psi_L(T') \leftarrow \emptyset, \forall T' \in \mathds{N}^+$; $E' \leftarrow \emptyset$; $m \leftarrow \sum_k S(k)$ \\
$AE(1) \leftarrow 0$; $AE(i) \leftarrow 1, \forall i = \{2, \cdots, n\}$; $\Psi_{L}(0) \leftarrow \{v_{1}\} $ \label{line:nedgestart}\\ 
\While {$\operatorname{sum}(AE) < m$}{
$a \sim \operatorname{discrete-uniform}(\{2 , \cdots n\})$; $AE(a) \leftarrow AE(a) + 1$\label{line:nedgeend}\\ 
% $AE(a) \leftarrow AE(a) + 1$ where $a$ is sampled from $\{2 , \cdots n\}$ uniformly at random.
}

\While{$idx < n$}{   
    % \state $K \leftarrow T^{\beta} \times C$ \Comment{Number of new nodes in the current level}\label{line:newnodes}\\ 
    $T \leftarrow T + 1 $\Comment{{level in the hierarchy}}  \\
    $\Psi_{L}(T) \leftarrow\{v_{(idx + i)}\}_{1 \leq i \leq \min(CT^{\beta}, n - idx)}$ \label{line:currentlevel}
    \Comment{{node set at level $T$}} 
    \\
    \For {$i = 1 \ \textbf{to} \  \min (CT^{\beta}, n - idx) $}{
        $idx \leftarrow idx + 1$ \\ 
        \For {$j = 1 \ \textbf{to} \ AE(idx)$ }{
            $e' \leftarrow \{v_{idx}\}$; $s \sim S$; $q \sim \operatorname{uniform}(0, 1)$ \label{line:sample_prep} \\
            \If {$q$ < $p$} {
                $e'{\leftarrow}$ \textbf{\texttt{IntraCommunityGenerate}}($e'{,}idx{,}C{,}T{,}s{,}\Psi_{L}$) \\
                }
            \If {$\lvert e'\vert$ < s} {
                $e' \leftarrow$ \textbf{\texttt{HierarchicalGenerate}}($e', T, s, \Psi_{L}$)
                }
            $E' \leftarrow E' \cup \{ e' \}$
            }
        }
    }
\textbf{return} $G' = (V' = \{v_{1} , \cdots , v_{n}\}, E')$  \\ 
 \nlnonumber
\nonumber \hrulefill \\
\setcounter{AlgoLine}{0}
\nlnonumber
\SetKwProg{myproc}{\texttt{IntraCommunityGenerate}}{($e', {idx}, C, T, s, \Psi_L$)}{}~\label{subalgo:intracom}
  \myproc{}{
  ${idx'} = C \times \ceil[\big]{({idx}-2)/C} + 1$ \Comment{beginning index of community} \label{line:intracombeg}\\ 
  $V_{C} \leftarrow \Psi_L(T) \cap \{v_{({idx'} + 1)}, \cdots ,v_{({idx'} + C)}\} \setminus e'$ \label{line:intracomend}\Comment{community}\\
  % \Comment{community nodes} \\
  $V' \leftarrow $ uniformly sample $\min(s - 1, |V_C|)$ nodes from $V_{C}$ \\ 
  % $\min(\lvert V_{C}\vert , s - \lvert e'\vert)$ nodes from $V_{C}$ \\ 
  \Return $e' \cup V'$ \\
  }  
\setcounter{AlgoLine}{0}
\nlnonumber
\SetKwProg{myproce}{\texttt{HierarchicalGenerate}}{($e', T, s, \Psi_{L})$}{}~\label{subalgo:hier}
  \myproce{}{ 
  \While{$\lvert e'\vert < s$}{
    $\ell \leftarrow $ sample a level from $[0, 1, \cdots , T] $ proportional to $[\lvert \Psi_{L}(0)\vert, \alpha^{-1}\lvert \Psi_{L}(1)\vert , \cdots , \alpha^{-T}\lvert \Psi_{L}(T)\vert]$ respectively \label{line:firstsample}\\
    $v' \leftarrow $ sample a node from $\Psi_{L}(\ell)$ uniformly at random \label{line:secondsample}\\ 
    $e' \leftarrow e' \cup \{v'\}$
    }
    % \state \textbf{return} $e'$ \\
    \Return $e'$ \\
  }  
\end{algorithm}
% \end{figure}

==> main_complex.tex <==
\begin{table*}[t!]
\caption{Runtime (sec.) and memory consumption (MB) of five generators {for approximating} 12 real-world hypergraphs. 
{Note that \generator achieves the fastest generation time for all six hypergraphs with $\vert V \vert \geq 10^4$ (\textit{coauthorship} and \textit{q\&a}), and it exhibits the lowest memory consumption in four out of the six hypergraphs.
For each hypergraph, the best results are colored. `-' indicates that the generation process either exceeds the time limit of 12 hours or encounters an out-of-memory issue.}} \label{tab:gentimeandmemory}
    \centering
    \scalebox{0.75}{
    \renewcommand{\arraystretch}{0.92}
        \centering
        \begin{tabular}{c | c| c c c |c c c| c c |c c |c c | c}
            \toprule
            \multirow{2}{*}{\textbf{Statistic}} & \multirow{2}{*}{\textbf{Generator}} & \multicolumn{3}{c|}{coauthorship} & \multicolumn{3}{c|}{q\&a} & 
            \multicolumn{2}{c|}{email} & \multicolumn{2}{c|}{ndc} &  \multicolumn{2}{c|}{contact} & Average \\
            & & dblp & geology & history & ubuntu & math & server & enron & eu & classes & substances & high & primary & ranking \\
            \midrule
            \midrule
            \multirow{6}{*}{\makecell{\textbf{Runtime} \\ 
            \textbf{(sec.)}}} &\textbf{\generator} & \goat 4.07 & \goat 2.39 & \goat 1.86 & \goat 0.39 & \goat 0.33 & \goat 0.63 & 0.04 & 0.18 & 0.04 & \goat 0.09 & 0.10 & 0.18  & 1.7 \goat\\
            %\midrule
            \cmidrule{2-15}
            
            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & 374.51 & - & - & 5.02 & 5011.84 & 1155.00 & - & 2.29 & 4.56 & 5.0\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 226.79 & 114.24 & 53.48 & 12.78 & 17.23 & 3.15 & 0.05 & \goat 0.09 & 0.32 & 0.10 & \goat 0.02 & \goat 0.02 & 2.7\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 19.07 & 9.57 & 2.24 & 0.57 & 0.45 & 1.14 & \goat 0.01 & 0.14 & \goat 0.01 & 0.10 & 0.06 & 0.04 & 1.8\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 1322.6 & 611.91 & 160.75 & 12.08 & 1.00 & 23.46 & 0.06 & 2.74 & 0.29 & 3.92 & 0.26 & 0.51 & 3.7\\
            \midrule 
            \midrule 
            
            \multirow{6}{*}{\makecell{\textbf{Memory} \\ \textbf{consumption} \\ 
            \textbf{(MB)}}} &\textbf{\generator} & \goattwo 1535 & \goattwo 761 & \goattwo 325 & 90 & \goattwo 36 & 129 & 2 & 3 & \goattwo 2 & 11 & 11 & 23 & 2.0 \goattwo\\
            \cmidrule{2-15}

            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & \goattwo 21 & - & - & 76 & 60169 & 21351 & - & 2 & 2 & 4.2\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 3307 & 1655 & 739 & 107 & 147 & \goattwo 26 & \goattwo 1 & \goattwo 2 & 4 & \goattwo 1 & \goattwo 1 & \goattwo 1 & 2.0 \goattwo \\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 3197 & 1498 & 529 & 134 & 86 & 204 & 11 & 32 & 15 & 41 & 12 & 11 & 3.1\\
            
            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 5042 & 3005 & 1901 & 591 & 110 & 321 & 9 & 39 & 14 & 412 & 10 & 18 & 3.8\\
            
            \bottomrule
        \end{tabular}
        }
\end{table*}

==> main_res.tex <==
\begin{table*}[t!]
\vspace{-2mm}
\caption{Hypergraph transitivity $T(G)$ and D-statistic {between} hyperwedge transitivity $\mathcal{T}(w)$ distributions {in} the real-world hypergraphs and the generated ones.
% : Real-world, \generator, HyperCL, HyperFF, HyperLAP, and HyperLAP+. 
Among six generators, \generator reproduces $T(G)$ and distribution of $\mathcal{T}(w)$ most accurately.
%\textcolor{limegreen} cell implies minimum gap from real-world $T(G)$, and \textcolor{dodgerblue} cell implies minimum D-stat
The best reproduction results on each dataset are colored, and `*' indicates that the value is less than $10^{-3}$.
{`-' indicates that the generation process either exceeds the time limit of 12 hours or encounters an out-of-memory issue.}
} \label{tab:genobservation1}
\vspace{-1mm}
    \centering
    \scalebox{0.8}{
    \renewcommand{\arraystretch}{0.9}
        \centering
        \begin{tabular}{c | c| c c |c c |c c| c c c| c c c | c}
            \toprule
            \multirow{2}{*}{\textbf{Statistic}} & \multirow{2}{*}{\textbf{Generator}} &  \multicolumn{2}{c|}{email} & \multicolumn{2}{c|}{NDC} & \multicolumn{2}{c|}{contact} & \multicolumn{3}{c|}{coauthorship} & \multicolumn{3}{c|}{q\&a} & Average \\
            & & enron & eu & classes & substances & high & primary & dblp & geology & history & ubuntu & server & math  & ranking \\
            \midrule
            \midrule
            \multirow{7}{*}{\makecell{ \textbf{Hypergraph} \\ \textbf{transitivity} \\ \textbf{$T(G)$}}}&\textbf{Real World} & 0.195 & 0.125 & 0.052 & 0.019 & 0.345 & 0.336 & 0.007 & 0.005 & 0.002 & 0.005 & 0.005 & 0.025 & Real\\
            %\midrule 
            \cmidrule{2-15}
            
            &\textbf{\generator} & \goat 0.192 &  0.124 & \goat 0.052 & \goat 0.019 & \goat 0.344 & \goat 0.334 & \goat 0.007 & \goat 0.005 & \goat 0.002 & \goat 0.004 & \goat 0.004 & \goat 0.025  & \goat 1.08\\
            %\midrule
            \cmidrule{2-15}
            
            &\textbf{HyperCL}~\cite{lee2021hyperedges} & 0.078 & 0.053 & 0.008 & 0.005 & 0.119 & 0.223 & 0.000* & 0.000* & 0.000* & 0.014 & 0.017 & 0.040  &  4.08\\
            
            &\textbf{HyperPA}~\cite{do2020structural} & 0.090 & 0.110 & 0.070 & - & 0.121 & 0.153 & - & - & - & 0.003 & - & - & 4.75\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 0.176 & \goat 0.125 & 0.006 & 0.003 & 0.006 & 0.007 & 0.047 & 0.048 & 0.048 & 0.051 & 0.050 & 0.054 &  4.83\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 0.123 & 0.085 & 0.008 & 0.008 & 0.220 & 0.301 & 0.001 & 0.000* & 0.000* & 0.016 & 0.015 & 0.004 & 3.25\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 0.231 & 0.144 & 0.026 & 0.016 & 0.322 & 0.338 & 0.042 & 0.019 & 0.005 & 0.029 & 0.023 & 0.007 & 3.54\\
            \midrule 
            \midrule 
            
            \multirow{6}{*}{\makecell{\textbf{D-Statistic from} \\ \textbf{real-world $\mathcal{T}(w)$} \\ 
            \textbf{distribution}}} &\textbf{\generator} & 0.137 & 0.186 & 0.208 & 0.187 & \goattwo 0.101 & \goattwo 0.099 & \goattwo 0.111 & 0.197 & \goattwo 0.066 & 0.035 & 0.170 & 0.101 & \goattwo 2.25\\
            \cmidrule{2-15}
            &\textbf{HyperCL} & 0.285 & 0.285 & 0.395 & 0.482 & 0.372 & 0.243 & 0.239 & 0.385 & 0.113 & \goattwo 0.020 & 0.054 & 0.084 & 3.75 \\
            &\textbf{HyperPA}~\cite{do2020structural} & 0.235 & 0.319 & 0.410 & - & 0.360 & 0.319 & - & - & - & 0.034 & - & - & 5.25\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & \goattwo 0.094 & \goattwo 0.158 & 0.638 & 0.831 & 0.631 & 0.699 & 0.126 & \goattwo 0.131 & 0.290 & 0.354 & 0.215 & 0.087 & 3.75\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 0.191 & 0.178 & 0.369 & 0.326 & 0.223 & 0.124 & 0.150 & 0.265 & 0.089 & 0.021 & \goattwo 0.051 & \goattwo 0.051 & 2.50\\
            
            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 0.262 & 0.244 & \goattwo 0.175 & \goattwo 0.185 & 0.166 & 0.180 & 0.509 & 0.405 & 0.119 & 0.061 & 0.104 & 0.184 & 3.23\\
            
            \bottomrule
        \end{tabular}
        }
\end{table*}

==> tables/Email_EU_AP.tex <==
\begin{table}[t!]
    \centering
    \caption{AP (in \%) in the detection of dynamic anomaly nodes in the two synthetic datasets.
    In both datasets, \method performs best compared to unsupervised methods in AP.\label{tab:Email_AP}
    }
    \setlength{\tabcolsep}{2.5pt}
    %\setlength{\tabcolsep}{5pt}
    %\setlength\aboverulesep{2pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cc}
            \toprule
            Method & Synthetic-Hijack & Synthetic-New  \\
            \midrule
            \midrule
                Random Guess & 6.61 $\pm$ 0.07 & 6.63 $\pm$ 0.01 \\
            \midrule
                \SedanSpot~\citep{eswaran2018sedanspot}   & 13.95 $\pm$ 1.53   & 15.17 $\pm$ 0.13     \\ \MIDAS~\citep{bhatia2020midas}  & \ul{17.96 $\pm$ 2.56}   & \ul{18.29 $\pm$ 3.18}     \\                \FFADE~\citep{chang2021f}  & 6.57 $\pm$ 0.00   & 6.58 $\pm$ 0.00        \\               \Anoedgel~\citep{bhatia2021sketch}            & 8.20 $\pm$ 0.47   & 8.40 $\pm$ 0.63    \\
            \midrule 
            \rule{0pt}{8pt}
                \tb{\method}
                 &\textbf{69.69 $\pm$ 7.33}  & \textbf{74.46 $\pm$ 6.16} \\
            \bottomrule
        \end{tabular}
}
    \normalsize
\end{table}

==> tables/Email_baselines.tex <==
\begin{figure*}[t!]
    \begin{subfigure}{0.45\textwidth}
        \centering
        %\setlength\aboverulesep{0.5pt}
        %\setlength\belowrulesep{0.5pt}
        \includegraphics[width=\linewidth]{figs/Email_MIDAS_all_scenario.png}
        \caption*{{(a) Type Analysis of MIDAS}}
        \label{fig:sub1}
        \vspace{0.02\textwidth}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \centering
        %\setlength\aboverulesep{0.5pt}
        %\setlength\belowrulesep{0.5pt}
        \includegraphics[width=\linewidth]{figs/Email_Sedanspot_all_scenario.png}
        \caption*{(b) Type Analysis of SedanSpot}
        \label{fig:sub2}
        \vspace{0.02\textwidth}
    \end{subfigure}
    \caption{ \label{fig:Email_baseline_test}
         For both (a) and (b), the above figures show the distribution of anomaly scores predicted by each baseline for each class in the two synthetic datasets (utilizing kernel density estimation).
         The below figures show the anomaly scores predicted by each baseline over time for each class in both datasets.
         We display the anomaly scores of \MIDAS on a log scale.
    }
\end{figure*}


==> tables/Email_hide_AUC.tex <==
\begin{table}[H]
    \centering
    \caption{AUC (in \%) in the detection of dynamic anomaly nodes in Synthetic-Hide and Synthetic-New.
    In both datasets, \method performs best compared to unsupervised methods in AUC.\label{tab:Email_hide}
    }
    \setlength{\tabcolsep}{2.5pt}
    %\setlength{\tabcolsep}{5pt}
    %\setlength\aboverulesep{2pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cc}
            \toprule
            Method & Synthetic-Hide & Synthetic-New  \\
            \midrule
            \midrule                \SedanSpot~\citep{eswaran2018sedanspot}   & 75.18 $\pm$ 2.12   & 78.05 $\pm$ 1.68     \\ \MIDAS~\citep{bhatia2020midas}  & \ul{81.78 $\pm$ 0.09}   & \ul{82.63 $\pm$ 0.07}     \\                \FFADE~\citep{chang2021f}  & 41.54 $\pm$ 0.00   & 48.73 $\pm$ 0.00        \\               \Anoedgel~\citep{bhatia2021sketch}            & 60.57 $\pm$ 2.11   & 61.86 $\pm$ 2.41    \\
            \midrule 
            \rule{0pt}{8pt}
                \tb{\method}
                 &\textbf{96.11 $\pm$ 3.31}  & \textbf{98.38 $\pm$ 1.09} \\
            \bottomrule
        \end{tabular}
}
    \normalsize
\end{table}

==> tables/Email_test_caption.tex <==

\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}            \caption{(a)} 
        \centering
        \includegraphics[width=\linewidth]{figs/Email_CLADE_hijack_pdf.png}
        \label{fig:subfig-a}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \caption{(b)} 
        \centering
        \includegraphics[width=\linewidth]{figs/Email_CLADE_new_pdf.png}
        \label{fig:subfig-b}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \caption{(c)}
        \centering
        \includegraphics[width=\linewidth]{figs/Email_CLADE_hijack_time.png}
        \label{fig:subfig-c}
    \end{subfigure}
    \begin{subfigure}{0.4\textwidth}
        \caption{(d)}
        \centering
        \includegraphics[width=\linewidth]{figs/Email_CLADE_new_time.png} 
        \label{fig:subfig-d}
    \end{subfigure}
    \caption{\label{fig:Email_test}
         (a) and (b) show the distribution of anomaly scores assigned by \method to instances of each node type in the two synthetic datasets (visualization is based on Gaussian kernel density estimation).
         (c) and (d) show the anomaly scores at each time period.
         Note that in all figures, \method clearly distinguishes anomalies from normal nodes.
         For results from several baseline methods, refer to Appendix~\ref{sec:app:exp:scenario}
         \red{[TODO: (a)]}}
    \label{fig:subplot-example}
\end{figure}

==> tables/Email_total.tex <==
\begin{figure}[!t]
    \begin{subfigure}{0.5\textwidth}
    \centering
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cc}
            \toprule
            Method & Email-EU-Hijack & Email-EU-New  \\
            \midrule
            \midrule
                \SedanSpot~\red{\citep{eswaran2018sedanspot}}   & 77.13 $\pm$ 2.21   & 78.05 $\pm$ 1.68     \\ \MIDAS~\red{\citep{bhatia2020midas}}  & \ul{81.80 $\pm$ 1.26}   & \ul{82.63 $\pm$ 0.07}     \\                \FFADE~\red{\citep{chang2021f}}  & 48.24 $\pm$ 0.00   & 48.16 $\pm$ 0.00        \\               \Anoedgel~\red{\citep{bhatia2021sketch}}            & 58.87 $\pm$ 2.47   & 61.86 $\pm$ 2.41    \\
            \midrule 
            \rule{0pt}{8pt}
                \tb{\method}
                 &\textbf{98.08 $\pm$ 1.02}  & \textbf{98.38 $\pm$ 1.09} \\
            \bottomrule
        \end{tabular}
        }
        \caption*{\red{(a) Performance of \method with baselines in anomaly scenarios}}
        \label{fig:sub1}
        \vspace{0.05\textwidth}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        %\setlength\aboverulesep{0.5pt}
        %\setlength\belowrulesep{0.5pt}
        \includegraphics[width=\linewidth]{figs/Email_CLADE_test_interval.png}
        \caption*{\red{(b) Analysis of \method in anomaly scenarios}}
        \label{fig:sub2}
    \end{subfigure}
    \caption{ \label{fig:Email_test}
         \red{(a) AUC (in \%) in the detection of dynamic anomaly nodes in the two injected Email-EU datasets. 
        The best and the second-best performances are highlighted in \textbf{boldface} and \ul{underlined}, respectively.
         (b) The above figures show the distribution of anomaly scores predicted by \method for each class in the two injected Email-EU datasets (utilizing Gaussian kernel density estimation).
         The below figures show the anomaly scores predicted by \method over time for each class in both datasets. The red bidirectional arrows indicate the range where anomalies have been injected.}
    }
\end{figure}


==> tables/Email_total_reverse.tex <==
\begin{figure}[!t]
    \begin{subfigure}{0.5\textwidth}
    \centering
    \setlength{\tabcolsep}{3pt}
    \scalebox{0.9}{
        \def\arraystretch{1}
        \begin{tabular}{l|ccc|c}
            \toprule
            Dataset & \SedanSpot & \MIDAS &  \Anoedgel & \method  \\
            \midrule
            \midrule                
            Email-EU-Hijack & 77.13 $\pm$ 2.21   & 81.80 $\pm$ 1.26 &  58.87 $\pm$ 2.47 & \textbf{98.08 $\pm$ 1.02}     \\ 
            Email-EU-New  & 78.05 $\pm$ 1.68   & 82.63 $\pm$ 0.07 &  61.86 $\pm$ 2.41 & \textbf{98.38 $\pm$ 1.09}    \\           
            \bottomrule
        \end{tabular}
        }
        \caption*{\red{(a) Performance of \method with baselines in anomaly scenarios}}
        \label{fig:sub1}
        \vspace{0.05\textwidth}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        %\setlength\aboverulesep{0.5pt}
        %\setlength\belowrulesep{0.5pt}
        \includegraphics[width=\linewidth]{figs/Email_CLADE_test_interval.png}
        \caption*{\red{(b) Analysis of \method in anomaly scenarios}}
        \label{fig:sub2}
    \end{subfigure}
    \caption{ \label{fig:Email_test}
         \red{(a) AUC (in \%) in the detection of dynamic anomaly nodes in the two injected Email-EU datasets. 
         To clarify, we exclude the baseline with AUC value below 0.5.
        The best performance is highlighted in \textbf{boldface}.
         (b) The above figures show the distribution of anomaly scores predicted by \method for each class in the two injected Email-EU datasets (utilizing Gaussian kernel density estimation).
         The below figures show the anomaly scores predicted by \method over time for each class in both datasets. The red bidirectional arrows indicate the range where anomalies have been injected.}
    }
\end{figure}


==> tables/Email_total_revision.tex <==
\begin{document}

\begin{figure}
\capbtabbox{%
   \centering
    \setlength{\tabcolsep}{3pt}
    \scalebox{0.9}{
        \def\arraystretch{1}
        \begin{tabular}{l|ccc|c}
            \toprule
            Dataset & \SedanSpot & \MIDAS &  \Anoedgel & \method  \\
            \midrule
            \midrule                
            Email-EU-Hijack & 77.13 $\pm$ 2.21   & 81.80 $\pm$ 1.26 &  58.87 $\pm$ 2.47 & \textbf{98.08 $\pm$ 1.02}     \\ 
            Email-EU-New  & 78.05 $\pm$ 1.68   & 82.63 $\pm$ 0.07 &  61.86 $\pm$ 2.41 & \textbf{98.38 $\pm$ 1.09}    \\           
            \bottomrule
        \end{tabular}
        }
        \caption*{\red{(a) Performance of \method with baselines in anomaly scenarios}}
        \label{fig:sub1}

\ffigbox{%
  \includegraphics[width=\linewidth]{example-image}%
}{%
  \caption{Neural Network: Confusion Matrix}%
  \label{fig:conMat_NN}%
}%
\capbtabbox{%
\begin{tabular}{|c|c|c|c|c|}
\hline
Year & 1 & 2 & 3 & 4 \\
\hline
\multicolumn{5}{c}{Neural Network} \\
\hline
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
Accuracy & 0.78 & 0.76 & 0.74 & 0.72 \\
\hline
\end{tabular}
}{%
  \caption{A table}%
}
\end{figure}

\end{document}

==> tables/accuracy.tex <==

% \begin{table*}[!t]
%     \setlength{\tabcolsep}{5pt}
%     \centering
%     \small
%     \scalebox{1}{
%         \begin{tabular}{clccccccccccc}
%             \toprule
%             & Method & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
%             \midrule
%             \midrule
%             \multirow{10}{*}{\rotatebox{90}{Supervised}} 
%                 & \MLP              & 60.32 $\pm$ 1.5   & 62.06 $\pm$ 2.3  & 76.27 $\pm$ 1.1        & 64.05 $\pm$ 1.4   & 81.18 $\pm$ 0.2   & 75.62 $\pm$ 9.5   & 79.19 $\pm$ 0.5       & 99.58 $\pm$ 0.3   & 65.17 $\pm$ 2.3   & 93.75 $\pm$ 0.6  & 12.5   \\
%                 & \GCN\!$^{\star}$  & 77.11 $\pm$ 1.8   & 66.07 $\pm$ 2.4  & 82.63 $\pm$ 0.6        & 73.66 $\pm$ 1.3   & 87.58 $\pm$ 0.2   & 36.79 $\pm$ 9.6   & OOM                   & 92.47 $\pm$ 0.9   & 71.17 $\pm$ 2.4   & 91.67 $\pm$ 0.2  & 11.7   \\
%                 & \GAT\!$^{\star}$  & 77.75 $\pm$ 2.1   & 67.62 $\pm$ 2.5  & 81.96 $\pm$ 0.7        & 74.52 $\pm$ 1.3   & 88.59 $\pm$ 0.1   & 36.48 $\pm$ 10.0  & OOM                   & OOM               & 70.94 $\pm$ 2.6   & 91.43 $\pm$ 0.3  & 11     \\
%                 & \HGNN             & 77.50 $\pm$ 1.8   & 66.16 $\pm$ 2.3  & 83.52 $\pm$ 0.7        & 74.38 $\pm$ 1.2   & 88.32 $\pm$ 0.3   & 78.58 $\pm$ 11.1  & 80.15 $\pm$ 0.3       & 98.59 $\pm$ 0.5   & 72.03 $\pm$ 2.4   & 92.23 $\pm$ 0.2  & 8.1    \\
%                 & \HyperConv        & 76.19 $\pm$ 2.1   & 64.12 $\pm$ 2.6  & 83.42 $\pm$ 0.6        & 73.52 $\pm$ 1.0   & 88.83 $\pm$ 0.2   & 62.53 $\pm$ 14.5  & 79.83 $\pm$ 0.4       & 97.56 $\pm$ 0.6   & 72.62 $\pm$ 2.6   & 91.84 $\pm$ 0.1  & 9.8    \\
%                 & \HNHN             & 76.21 $\pm$ 1.7   & 67.28 $\pm$ 2.2  & 80.97 $\pm$ 0.9        & 74.88 $\pm$ 1.6   & 86.71 $\pm$ 1.2   & 78.89 $\pm$ 10.2  & 79.51 $\pm$ 0.4       & 99.78 $\pm$ 0.1   & 71.45 $\pm$ 3.2   & 92.96 $\pm$ 0.2  & 8.9    \\
%                 & \HyperGCN         & 64.11 $\pm$ 7.4   & 59.92 $\pm$ 9.6  & 78.40 $\pm$ 9.2        & 60.65 $\pm$ 9.2   & 76.59 $\pm$ 7.6   & 40.86 $\pm$ 2.1   & 77.31 $\pm$ 6.0       & 48.26 $\pm$ 0.3   & 46.05 $\pm$ 3.9   & 69.23 $\pm$ 2.8  & 15.1   \\
%                 & \HyperSAGE        & 64.98 $\pm$ 5.3   & 52.43 $\pm$ 9.4  & 79.49 $\pm$ 8.7        & 64.59 $\pm$ 4.3   & 79.63 $\pm$ 8.6   & 40.86 $\pm$ 2.1   & OOT              & OOT          & OOT          & OOT         & 14.7   \\
%                 & \UniGCN           & 77.91 $\pm$ 1.9   & 66.40 $\pm$ 1.9  & \ul{84.08 $\pm$ 0.7}   & 77.30 $\pm$ 1.4   & 90.31 $\pm$ 0.2   & 72.10 $\pm$ 12.1  & \tb{80.24 $\pm$ 0.4}  & 98.84 $\pm$ 0.5   & 73.27 $\pm$ 2.7   & 94.62 $\pm$ 0.2  & 5.9    \\
%                 & \AllSet           & 76.21 $\pm$ 1.7   & 67.83 $\pm$ 1.8  & 82.85 $\pm$ 0.9        & 76.94 $\pm$ 1.3   & 90.07 $\pm$ 0.3   & 72.72 $\pm$ 11.8  & 79.90 $\pm$ 0.4       & 99.78 $\pm$ 0.1   & 75.09 $\pm$ 2.5   & 96.85 $\pm$ 0.2  & 6.2    \\
%             \midrule
%             \multirow{8}{*}{\rotatebox{90}{Unsupervised}}
%                 & \Nodetovec\!$^{\star}$    & 70.99 $\pm$ 1.4   & 53.85 $\pm$ 1.9   & 78.75 $\pm$ 0.9   & 58.50 $\pm$ 2.1   & 72.09 $\pm$ 0.3   & 17.02 $\pm$ 4.1   & 63.35 $\pm$ 1.7   & 88.16 $\pm$ 0.8   & 67.72 $\pm$ 2.1   & 84.94 $\pm$ 0.4   & 15.6  \\
%                 & \DGI\!$^{\star}$          & 78.17 $\pm$ 1.4   & 68.81 $\pm$ 1.8   & 80.83 $\pm$ 0.6   & 76.94 $\pm$ 1.1   & 88.00 $\pm$ 0.2   & 36.54 $\pm$ 9.7   & OOM               & OOM               & 72.01 $\pm$ 2.5   & 92.18 $\pm$ 0.2   & 9.3   \\
%                 & \GRACE\!$^{\star}$        & 79.11 $\pm$ 1.7   & 68.65 $\pm$ 1.7   & 80.08 $\pm$ 0.7   & 76.59 $\pm$ 1.0   & OOM               & 37.07 $\pm$ 9.3   & OOM               & OOM               & 70.51 $\pm$ 2.4   & 90.68 $\pm$ 0.3   & 10.4  \\
%                 & \HHGR                     & 78.08 $\pm$ 1.7   & 68.21 $\pm$ 1.8   & 82.13 $\pm$ 0.6   & 78.15 $\pm$ 1.1   & 88.69 $\pm$ 0.2   & 80.06 $\pm$ 11.1  & 79.75 $\pm$ 0.3   & 97.15 $\pm$ 0.5   & 73.95 $\pm$ 2.4   & 93.26 $\pm$ 0.2   & 6.8   \\
%                 \cmidrule{2-13}
%                 & \RandomInit           & 63.62 $\pm$ 3.1       & 60.44 $\pm$ 2.5       & 67.49 $\pm$ 2.2       & 66.27 $\pm$ 2.2       & 76.57 $\pm$ 0.6       & 78.43 $\pm$ 11.0      & 77.14 $\pm$ 0.6       & 97.40 $\pm$ 0.6       & 74.39 $\pm$ 2.6       & 96.29 $\pm$ 0.3       & 11.9      \\
%                 & \tb{\methodN}         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5       & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 79.94 $\pm$ 11.1      & \ul{80.18 $\pm$ 0.2}  & 99.76 $\pm$ 0.2       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 3.4       \\
%                 & \tb{\methodNE}        & \ul{81.45 $\pm$ 1.2}  & \ul{71.38 $\pm$ 1.2}  & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & \ul{80.19 $\pm$ 11.1} & \ul{80.18 $\pm$ 0.2}  & \ul{99.81 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & \ul{97.02 $\pm$ 0.1}  & \ul{2}    \\
%                 & \tb{\method}          & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.2}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \tb{80.25 $\pm$ 11.2} & 80.14 $\pm$ 0.2       & \tb{99.83 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.5}  \\
%             \bottomrule
%         \end{tabular}
%     }
%     \normalsize
%     \vspace{-2mm}
%     \caption{Node classification accuracy and standard deviations. 
%     Graph methods, marked as $\star$, are applied after converting hypergraphs to graphs via clique expansion.
%     For each dataset, the best and the second-best performances are highlighted in boldface and underlined, respectively.
%     A.R. denotes average rank, OOT denotes cases where results are not obtained within 24 hours, and OOM indicates out of memory on a 24GB GPU.
%     In most cases, \method outperforms all others, including the supervised ones.
%     }
%     \label{tab:accuracy}
% \end{table*}





\begin{table*}[!t]
    \setlength{\tabcolsep}{5pt}
    \setlength\aboverulesep{0.5pt}
    \centering
    \small
    \scalebox{1}{
        \begin{tabular}{clcccccccc}
            \toprule
            & Method & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            \midrule
            \midrule
            \multirow{10}{*}{\rotatebox{90}{Supervised}} 
                & \MLP              & 60.32 $\pm$ 1.5   & 62.06 $\pm$ 2.3  & 76.27 $\pm$ 1.1        & 64.05 $\pm$ 1.4   & 81.18 $\pm$ 0.2   & 65.17 $\pm$ 2.3   & 93.75 $\pm$ 0.6   & 14.4   \\
                & \GCN\!$^{\star}$  & 77.11 $\pm$ 1.8   & 66.07 $\pm$ 2.4  & 82.63 $\pm$ 0.6        & 73.66 $\pm$ 1.3   & 87.58 $\pm$ 0.2   & 71.17 $\pm$ 2.4   & 91.67 $\pm$ 0.2   & 11.1   \\
                & \GAT\!$^{\star}$  & 77.75 $\pm$ 2.1   & 67.62 $\pm$ 2.5  & 81.96 $\pm$ 0.7        & 74.52 $\pm$ 1.3   & 88.59 $\pm$ 0.1   & 70.94 $\pm$ 2.6   & 91.43 $\pm$ 0.3   & 10.1     \\
                & \HGNN             & 77.50 $\pm$ 1.8   & 66.16 $\pm$ 2.3  & 83.52 $\pm$ 0.7        & 74.38 $\pm$ 1.2   & 88.32 $\pm$ 0.3   & 72.03 $\pm$ 2.4   & 92.23 $\pm$ 0.2   & 9    \\
                & \HyperConv        & 76.19 $\pm$ 2.1   & 64.12 $\pm$ 2.6  & 83.42 $\pm$ 0.6        & 73.52 $\pm$ 1.0   & 88.83 $\pm$ 0.2   & 72.62 $\pm$ 2.6   & 91.84 $\pm$ 0.1   & 10.1    \\
                & \HNHN             & 76.21 $\pm$ 1.7   & 67.28 $\pm$ 2.2  & 80.97 $\pm$ 0.9        & 74.88 $\pm$ 1.6   & 86.71 $\pm$ 1.2   & 71.45 $\pm$ 3.2   & 92.96 $\pm$ 0.2   & 10.3    \\
                & \HyperGCN         & 64.11 $\pm$ 7.4   & 59.92 $\pm$ 9.6  & 78.40 $\pm$ 9.2        & 60.65 $\pm$ 9.2   & 76.59 $\pm$ 7.6   & 46.05 $\pm$ 3.9   & 69.23 $\pm$ 2.8   & 16.3   \\
                & \HyperSAGE        & 64.98 $\pm$ 5.3   & 52.43 $\pm$ 9.4  & 79.49 $\pm$ 8.7        & 64.59 $\pm$ 4.3   & 79.63 $\pm$ 8.6   & OOT               & OOT               & 16   \\
                & \UniGCN           & 77.91 $\pm$ 1.9   & 66.40 $\pm$ 1.9  & \ul{84.08 $\pm$ 0.7}   & 77.30 $\pm$ 1.4   & 90.31 $\pm$ 0.2   & 73.27 $\pm$ 2.7   & 94.62 $\pm$ 0.2   & 5.9    \\
                & \AllSet           & 76.21 $\pm$ 1.7   & 67.83 $\pm$ 1.8  & 82.85 $\pm$ 0.9        & 76.94 $\pm$ 1.3   & 90.07 $\pm$ 0.3   & 75.09 $\pm$ 2.5   & 96.85 $\pm$ 0.2   & 6.3    \\
            \midrule
            \multirow{8}{*}{\rotatebox{90}{Unsupervised}}
                & \Nodetovec\!$^{\star}$    & 70.99 $\pm$ 1.4   & 53.85 $\pm$ 1.9   & 78.75 $\pm$ 0.9   & 58.50 $\pm$ 2.1   & 72.09 $\pm$ 0.3   & 67.72 $\pm$ 2.1   & 84.94 $\pm$ 0.4   & 16  \\
                & \DGI\!$^{\star}$          & 78.17 $\pm$ 1.4   & 68.81 $\pm$ 1.8   & 80.83 $\pm$ 0.6   & 76.94 $\pm$ 1.1   & 88.00 $\pm$ 0.2   & 72.01 $\pm$ 2.5   & 92.18 $\pm$ 0.2   & 8.3   \\
                & \GRACE\!$^{\star}$        & 79.11 $\pm$ 1.7   & 68.65 $\pm$ 1.7   & 80.08 $\pm$ 0.7   & 76.59 $\pm$ 1.0   & OOM               & 70.51 $\pm$ 2.4   & 90.68 $\pm$ 0.3   & 11  \\
                & \HHGR                     & 78.08 $\pm$ 1.7   & 68.21 $\pm$ 1.8   & 82.13 $\pm$ 0.6   & 78.15 $\pm$ 1.1   & 88.69 $\pm$ 0.2   & 73.95 $\pm$ 2.4   & 93.26 $\pm$ 0.2   & 6.6   \\
                \cmidrule{2-10}
                & \RandomInit           & 63.62 $\pm$ 3.1       & 60.44 $\pm$ 2.5       & 67.49 $\pm$ 2.2       & 66.27 $\pm$ 2.2       & 76.57 $\pm$ 0.6       & 74.39 $\pm$ 2.6       & 96.29 $\pm$ 0.3       & 12.9      \\
                & \tb{\methodN}         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5       & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 3.3       \\
                & \tb{\methodNE}        & \ul{81.45 $\pm$ 1.2}  & \ul{71.38 $\pm$ 1.2}  & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & \ul{97.02 $\pm$ 0.1}  & \ul{2}    \\
                & \tb{\method}          & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.2}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.1}  \\
            \bottomrule
        \end{tabular}
    }
    \normalsize
    % \vspace{-2mm}
    \caption{Node classification accuracy and standard deviations. 
    Graph methods, marked as $\star$, are applied after converting hypergraphs to graphs via clique expansion.
    For each dataset, the best and the second-best performances are highlighted in boldface and underlined, respectively.
    A.R. denotes average rank, OOT denotes cases where results are not obtained within 24 hours, and OOM indicates out of memory on a 24GB GPU.
    In most cases, \method outperforms all others, including the supervised ones.
    }
    \label{tab:accuracy}
\end{table*}

==> tables/accuracy2.tex <==
\begin{table*}
    % \vspace{-2mm}
    \caption{Node classification accuracy in percentage along with standard deviations. 
    Graph algorithms, marked as $\star$, are applied after converting hypergraphs to graphs via clique expansion.
    For each dataset, the highest and the second-highest performance is highlighted in \textbf{boldface} and \underline{underlined}, respectively.
    A.R. denotes average rank, Time-out represents cases where results are not obtained within 24 hours, and OOM indicates out of memory on a 24GB GPU. 
    % Note that only the listed datasets are used to compute average rank.
    }
    \label{tab:accuracy2}
    \centering
    \scalebox{0.8}{
        \begin{tabular}{clcccccc}
            \toprule
            % \multirow{2}{*}{} & \multirow{2}{*}[-1mm]{Method} & \multicolumn{3}{c}{Co-citation Data} & \multicolumn{2}{c}{Co-authorship Data} & \multirow{2}{*}[-1mm]{A.R.$\downarrow$} \\
            & Method & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            % \cmidrule(lr){3-5} \cmidrule(lr){6-7}
            % & & Cora & Citeseer & Pubmed & Cora & DBLP \\
            \midrule
            \midrule
            \multirow{10}{*}{\rotatebox{90}{Supervised}} 
                & \MLP              & 75.62 $\pm$ 9.47  & 79.19 $\pm$ 0.45  & 99.58 $\pm$ 0.29  & 65.17 $\pm$ 2.32  & 93.75 $\pm$ 0.61  & 8.8   \\
                & \GCN\!$^{\star}$  & 36.79 $\pm$ 9.59  & OOM               & 92.47 $\pm$ 0.89  & 71.17 $\pm$ 2.36  & 91.67 $\pm$ 0.21  & 13    \\
                & \GAT\!$^{\star}$  & 36.48 $\pm$ 10.0  & OOM               & OOM               & 70.94 $\pm$ 2.55  & 91.43 $\pm$ 0.26  & 14.7  \\
                & \HGNN             & 78.58 $\pm$ 11.1  & 80.15 $\pm$ 0.25  & 98.59 $\pm$ 0.48  & 72.03 $\pm$ 2.41  & 92.23 $\pm$ 0.16  & 7     \\
                & \HyperConv        & 62.53 $\pm$ 14.5  & 79.83 $\pm$ 0.36  & 97.56 $\pm$ 0.64  & 72.62 $\pm$ 2.64  & 91.84 $\pm$ 0.14  & 9.4   \\
                & \HNHN             & 78.89 $\pm$ 10.2  & 79.51 $\pm$ 0.43  & \textbf{99.78 $\pm$ 0.10}  & 71.45 $\pm$ 3.16  & 92.96 $\pm$ 0.17  & 7     \\
                & \HyperGCN         & 40.86 $\pm$ 2.10  & 77.31 $\pm$ 6.04  & 48.26 $\pm$ 0.26  & 46.05 $\pm$ 3.91  & 69.23 $\pm$ 2.83  & 14.2  \\
                & \HyperSAGE        & 40.86 $\pm$ 2.10  & Time-out          & Time-out          & Time-out          & Time-out          & -     \\
                & \UniGCN           & 72.10 $\pm$ 12.1  & \textbf{80.24 $\pm$ 0.36}  & 98.84 $\pm$ 0.53  & 73.27 $\pm$ 2.69  & 94.62 $\pm$ 0.19  & 6.2   \\
                & \AllSet           & 72.72 $\pm$ 11.8  & 79.90 $\pm$ 0.43  & \underline{99.78 $\pm$ 0.13}  & 75.09 $\pm$ 2.50  & 96.85 $\pm$ 0.21  & 4.8   \\
            \midrule
            \multirow{8}{*}{\rotatebox{90}{Unsupervised}}
                & \Nodetovec\!$^{\star}$  & 17.02 $\pm$ 4.12  & 63.35 $\pm$ 1.74    & 88.16 $\pm$ 0.77  & 67.72 $\pm$ 2.13  & 84.94 $\pm$ 0.44  & 15    \\
                & \DGI\!$^{\star}$        & 36.54 $\pm$ 9.67  & OOM                 & OOM               & 72.01 $\pm$ 2.51  & 92.18 $\pm$ 0.20  & 12.3  \\
                & \GRACE\!$^{\star}$      & 37.07 $\pm$ 9.30  & OOM                 & OOM               & 70.51 $\pm$ 2.38  & 90.68 $\pm$ 0.25  & 14.3  \\
                & \HHGR                 & \underline{80.06 $\pm$ 11.1}  & 79.75 $\pm$ 0.32      & 97.15 $\pm$ 0.49  & 73.95 $\pm$ 2.44  & 93.26 $\pm$ 0.18  & 7.2   \\
                \cmidrule{2-8}
                & \RandomInit           & 78.43 $\pm$ 11.0  & 77.14 $\pm$ 0.58  & 97.40 $\pm$ 0.58  & 74.39 $\pm$ 2.57  & 96.29 $\pm$ 0.28  & 7.8   \\
                & \textbf{\methodN}     & 79.77 $\pm$ 10.9  & 80.14 $\pm$ 0.23  & 99.54 $\pm$ 0.23  & 75.11 $\pm$ 2.52  & 97.01 $\pm$ 0.15  & 4.2   \\
                & \textbf{\methodNE}    & 79.99 $\pm$ 10.9  & 80.17 $\pm$ 0.22  & 99.65 $\pm$ 0.19  & \underline{75.14 $\pm$ 2.51}  & \underline{97.02 $\pm$ 0.14}  & \underline{2.6}   \\
                & \textbf{\method}      & \textbf{80.11 $\pm$ 11.1}  & 80.12 $\pm$ 0.20  & 99.67 $\pm$ 0.19  & \textbf{75.17 $\pm$ 2.49}  & \textbf{97.08 $\pm$ 0.13}  & \textbf{2.2}   \\
            \bottomrule
        \end{tabular}
    }
\end{table*}

==> tables/anomaly_detection_AP.tex <==
\begin{table}[t] % command h keeps table in the current position!
    \centering
    \caption{AP (in \%) in the detection of dynamic anomaly nodes. The first method randomly assigns anomaly scores from 0 to 1, and the next four methods are rule-based models, and the others are based on representation learning. 
    For each dataset, the best and the second-best performances are highlighted in \textbf{boldface} and \ul{underlined}, respectively.\label{tab:AP}
    }
    \setlength{\tabcolsep}{2.5pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cccc}
            \toprule
            Method & Wikipedia & Reddit & Bitcoin-alpha & Bitcoin-OTC  \\
            \midrule
            \midrule
                Random Guess & 0.22 $\pm$ 0.05 & 0.09 $\pm$ 0.01 & 8.96 $\pm$ 0.53 & 6.37 $\pm$ 0.28 \\
            \midrule
                \SedanSpot~\citep{eswaran2018sedanspot}  & 0.66 $\pm$ 0.06   & 0.09 $\pm$ 0.00  & 12.99 $\pm$ 0.06        & 16.14 $\pm$ 0.01     \\
                \MIDAS~\citep{bhatia2020midas}  & 0.41 $\pm$ 0.02   & 0.12 $\pm$ 0.00  & 12.99 $\pm$ 0.06        & 16.14 $\pm$ 0.01    \\
                \FFADE~\citep{chang2021f}  & 0.18 $\pm$ 0.00   & 0.09 $\pm$ 0.00  & 6.34 $\pm$ 0.00        & 8.80 $\pm$ 0.00      \\
                \Anoedgel~\citep{bhatia2021sketch}            & 0.18 $\pm$ 0.01   & 0.09 $\pm$ 0.00  & 12.52 $\pm$ 0.86        & 17.03 $\pm$ 0.11    \\
            \midrule 
                \JODIE~\citep{kumar2019predicting} & 1.40 $\pm$ 0.02   & 0.25 $\pm$ 0.05   & 14.31 $\pm$ 0.40  & 15.79 $\pm$ 0.11   \\
                \Dyrep~\citep{trivedi2019dyrep} & 1.53 $\pm$ 0.02   & 0.14 $\pm$ 0.01   & 8.41 $\pm$ 0.58   & 16.14 $\pm$ 1.74   \\
                \TGAT~\citep{xu2020inductive}  & 1.48 $\pm$ 0.14   & 0.27 $\pm$ 0.12   & 12.19 $\pm$ 0.13   & 18.81 $\pm$ 0.63   \\
                \TGN~\citep{tgn_icml_grl2020}  & 1.30 $\pm$ 0.04   & 0.19 $\pm$ 0.01   & 9.65 $\pm$ 0.40   & 19.87 $\pm$ 1.75     \\
                \SAD~\citep{tian2023sad}   & \tb{2.77 $\pm$ 0.91}       & \ul{0.28 $\pm$ 0.06}       & 12.55 $\pm$ 0.58       & 14.33 $\pm$ 0.88 \\
            \midrule
            \rule{0pt}{8pt}
                \tb{\method}
                 & 1.24 $\pm$ 0.14  & 
                 0.23 $\pm$ 0.02  & \tb{15.40 $\pm$ 0.19}  & \ul{20.21 $\pm$ 0.28}   \\
                 \rule{0pt}{10pt}
                \tb{\method-HP}        & \ul{1.56 $\pm$ 0.14}  & \tb{0.30 $\pm$ 0.05}  & \ul{14.86 $\pm$ 0.08}  & \tb{20.46 $\pm$ 0.06} \rule{0pt}{10pt}   \\
            \bottomrule
        \end{tabular}
}
    \normalsize
    % \vspace{-2mm}
\end{table}


%%sedanspot -> 5.5
%MIDAS -> 8.25
%FFADE  -> 9.75
%Anoedge  -> 8.75
%Jodie  -> 4
%Dyrep -> 4.5
%TGAT -> 4.5
%TGN  -> 3.25
%SAD  -> 4.75
%CLADE  -> 1.25

==> tables/backbone.tex <==
\begin{table}[!t]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lcc}
            \toprule
            Dataset & \method (with \HGNN) & \method (Proposed) \\
            \midrule
            \midrule
            Cora-C      & 81.03 $\pm$ 1.31  & \textbf{81.57 $\pm$ 1.12} \\
            Citeseer    & 71.97 $\pm$ 1.26  & \textbf{72.02 $\pm$ 1.16} \\
            Pubmed      & 83.80 $\pm$ 0.63  & \textbf{84.26 $\pm$ 0.62} \\
            Cora-A      & \textbf{82.22 $\pm$ 1.09}  & 82.15 $\pm$ 0.89 \\
            DBLP        & 90.93 $\pm$ 0.16  & \textbf{91.12 $\pm$ 0.11} \\
            Zoo         & 79.47 $\pm$ 11.0  & \textbf{80.25 $\pm$ 11.2} \\
            20News      & 79.93 $\pm$ 0.24  & \textbf{80.14 $\pm$ 0.19} \\
            Mushroom    & 98.93 $\pm$ 0.33  & \textbf{99.83 $\pm$ 0.13} \\
            NTU2012     & 74.63 $\pm$ 2.53  & \textbf{75.23 $\pm$ 2.45} \\
            ModelNet40  & \textbf{97.33 $\pm$ 0.14}  & 97.08 $\pm$ 0.13 \\
            \bottomrule
        \end{tabular}
    }
    \caption{
    The accuracy of two \method methods that use (1) \HGNN and (2) the mean pooling layer (proposed), respectively, as an encoder. 
    % \method using the mean pooling layer consistently and slightly outperforms the one using \HGNN as an encoder. 
    % This result justifies our choice of using the mean pooling layer as our backbone encoder.
    }
    \label{tab:backbone}
    \vspace{-2mm}
\end{table}

==> tables/comparison.tex <==



% \begin{table*}
%     \vspace{-1mm}
%     \setlength{\tabcolsep}{5pt}
%     \centering
%     \small
%     \scalebox{1}{
%         \begin{tabular}{cccccccccccccc}
%             \toprule
%             $\calL_{n}$ & $\calL_{g}$ & $\calL_{m}$ & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & Zoo & 20News & Mushroom & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
%             \midrule
%             \midrule
%             \ding{51}   & -         & -         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5*      & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 79.94 $\pm$ 11.1      & \tb{80.18 $\pm$ 0.2}  & 99.76 $\pm$ 0.2       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 3.8       \\
%             -           & \ding{51} & -         & 79.69 $\pm$ 1.6       & 71.02 $\pm$ 1.3*      & 80.20 $\pm$ 1.3       & 78.98 $\pm$ 1.4       & 88.60 $\pm$ 0.2       & 79.31 $\pm$ 10.7      & 79.35 $\pm$ 0.4       & 99.13 $\pm$ 0.3       & 74.41 $\pm$ 2.6       & 96.66 $\pm$ 0.2       & 5.7       \\
%             -           & -         & \ding{51} & 76.76 $\pm$ 1.8       & 63.98 $\pm$ 2.0       & 79.86 $\pm$ 0.9       & 76.77 $\pm$ 1.1       & 63.95 $\pm$ 7.2       & 79.80 $\pm$ 11.0      & 79.27 $\pm$ 0.3       & 94.87 $\pm$ 0.7       & 73.11 $\pm$ 2.8       & 96.57 $\pm$ 0.2       & 6.9       \\
%             \ding{51}   & \ding{51} & -         & \ul{81.45 $\pm$ 1.2}  & 71.38 $\pm$ 1.4       & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & 80.19 $\pm$ 11.1      & \tb{80.18 $\pm$ 0.2}  & \ul{99.81 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & 97.02 $\pm$ 0.1       & \ul{2.3}  \\
%             \ding{51}   & -         & \ding{51} & 80.49 $\pm$ 1.3       & 70.46 $\pm$ 1.5       & \ul{83.98 $\pm$ 0.7}  & 81.62 $\pm$ 1.0       & 90.75 $\pm$ 0.1       & 80.19 $\pm$ 11.1      & 80.15 $\pm$ 0.2       & 99.74 $\pm$ 0.2       & 75.12 $\pm$ 2.5       & \ul{97.03 $\pm$ 0.1}  & 3.6       \\
%             -           & \ding{51} & \ding{51} & 80.80 $\pm$ 1.1       & \ul{71.73 $\pm$ 1.4}  & 82.81 $\pm$ 0.7       & 80.24 $\pm$ 1.0       & 90.17 $\pm$ 0.1       & \ul{80.20 $\pm$ 11.1} & 79.29 $\pm$ 0.2       & 99.82 $\pm$ 0.1       & 73.76 $\pm$ 2.5       & 96.74 $\pm$ 0.1       & 4.1       \\
%             \ding{51}   & \ding{51} & \ding{51} & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.4}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \tb{80.25 $\pm$ 11.2} & 80.14 $\pm$ 0.2       & \tb{99.83 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.4}  \\
%             \bottomrule
%         \end{tabular}
%     }
%     \normalsize
%     \vspace{-2mm}
%     \caption{Comparison of node classification accuracy according to whether or not to use each type of contrast (i.e., $\calL_{n}$, $\calL_{g}$, and $\calL_{m}$). %(i.e., node, hyperedge, and membership-level contrast) 
%     Using all types of contrasts (i.e., node-, group-, and membership-level contrast) achieves the best performance in most cases as they are complementarily reinforcing each other.
%     }
%     \label{tab:comparison}
%     \vspace{-3mm}
% \end{table*}


\begin{table*}
    % \vspace{-1mm}
    \setlength{\tabcolsep}{5pt}
    \setlength\aboverulesep{0.5pt}
    \centering
    \small
    \scalebox{1}{
        \begin{tabular}{ccccccccccc}
            \toprule
            $\calL_{n}$ & $\calL_{g}$ & $\calL_{m}$ & Cora-C & Citeseer & Pubmed & Cora-A & DBLP & NTU2012 & ModelNet40 & A.R.$\downarrow$ \\
            \midrule
            \midrule
            \ding{51}   & -         & -         & 80.23 $\pm$ 1.2       & 70.28 $\pm$ 1.5*      & 83.44 $\pm$ 0.6       & 81.94 $\pm$ 1.1       & 90.88 $\pm$ 0.1       & 75.20 $\pm$ 2.6       & 97.01 $\pm$ 0.2       & 4      \\
            -           & \ding{51} & -         & 79.69 $\pm$ 1.6       & 71.02 $\pm$ 1.3*      & 80.20 $\pm$ 1.3       & 78.98 $\pm$ 1.4       & 88.60 $\pm$ 0.2       & 74.41 $\pm$ 2.6       & 96.66 $\pm$ 0.2       & 5.6       \\
            -           & -         & \ding{51} & 76.76 $\pm$ 1.8       & 63.98 $\pm$ 2.0       & 79.86 $\pm$ 0.9       & 76.77 $\pm$ 1.1       & 63.95 $\pm$ 7.2       & 73.11 $\pm$ 2.8       & 96.57 $\pm$ 0.2       & 7       \\
            \ding{51}   & \ding{51} & -         & \ul{81.45 $\pm$ 1.2}  & 71.38 $\pm$ 1.4       & 83.68 $\pm$ 0.7       & \ul{82.00 $\pm$ 1.0}  & \ul{90.94 $\pm$ 0.1}  & \tb{75.25 $\pm$ 2.5}  & 97.02 $\pm$ 0.1       & \ul{2.3}  \\
            \ding{51}   & -         & \ding{51} & 80.49 $\pm$ 1.3       & 70.46 $\pm$ 1.5       & \ul{83.98 $\pm$ 0.7}  & 81.62 $\pm$ 1.0       & 90.75 $\pm$ 0.1       & 75.12 $\pm$ 2.5       & \ul{97.03 $\pm$ 0.1}  & 3.6       \\
            -           & \ding{51} & \ding{51} & 80.80 $\pm$ 1.1       & \ul{71.73 $\pm$ 1.4}  & 82.81 $\pm$ 0.7       & 80.24 $\pm$ 1.0       & 90.17 $\pm$ 0.1       & 73.76 $\pm$ 2.5       & 96.74 $\pm$ 0.1       & 4.4       \\
            \ding{51}   & \ding{51} & \ding{51} & \tb{81.57 $\pm$ 1.1}  & \tb{72.02 $\pm$ 1.4}  & \tb{84.26 $\pm$ 0.6}  & \tb{82.15 $\pm$ 0.9}  & \tb{91.12 $\pm$ 0.1}  & \ul{75.23 $\pm$ 2.4}  & \tb{97.08 $\pm$ 0.1}  & \tb{1.1}  \\
            \bottomrule
        \end{tabular}
    }
    \normalsize
    % \vspace{-2mm}
    \caption{Comparison of node classification accuracy according to whether or not to use each type of contrast (i.e., $\calL_{n}$, $\calL_{g}$, and $\calL_{m}$). %(i.e., node, hyperedge, and membership-level contrast) 
    Using all types of contrasts (i.e., node-, group-, and membership-level contrast) achieves the best performance in most cases as they are complementarily reinforcing each other.
    }
    \label{tab:comparison}
    % \vspace{-3mm}
\end{table*}

==> tables/large_scale_time.tex <==
\begin{figure}[H]
    \centering
    \setlength\aboverulesep{0.5pt}
    \setlength\belowrulesep{0.5pt}
    \centering
    \includegraphics[width=1\linewidth]{figs/appendix_large_scale_time2.png} 
    \caption{
    \label{fig:Transportation} The left figure shows the increase in the inference time and the right figure shows the increase in the training time per epoch of \method with respect to the number of edges in a large-scale scenario. 
    }
\end{figure}


==> tables/rebutal_edge_SSL_analysis.tex <==
\begin{figure}[H]
    \centering
    \setlength\aboverulesep{0.5pt}
    \setlength\belowrulesep{0.5pt}
    \centering
    \includegraphics[width=1\linewidth]{figs/Edge_SSL_anlaysis.png} 
    \caption{
    \label{fig:Edge_SSL_analysis} The above figures show the frequency distribution of edges with the same node pair composition as those involving anomalous nodes compared to normal edges in Wikipedia and Reddit datasets. 
    }
\end{figure}




==> tables/rebuttal_DTDG_static.tex <==


\begin{table}[H]
    \centering
    \caption{\label{tab:DTDG_static} AUC (in \%) in the detection of dynamic anomaly nodes with DTDG-based baselines and a static graph-based baseline.}
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{0.95}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cccc}
            \toprule
            Method & Wikipedia & Reddit & Bitcoin-alpha & Bitcoin-OTC  \\
            \midrule
            \midrule
                DOMINANT~{\citep{ding2019deep}} & 67.15 $\pm$ 1.38   & 44.17 $\pm$ 0.53   & 54.21 $\pm$ 8.78  & 51.26 $\pm$ 0.01   \\
                STrGNN~{\citep{cai2021structural}} & 50.95 $\pm$ 0.46   & 53.30 $\pm$ 0.22   & 51.26 $\pm$ 0.01  & 47.85 $\pm$ 0.15   \\
                TADDY~{\citep{liu2021anomaly}} & 56.48 $\pm$ 1.41   & 54.54 $\pm$ 0.43   & 57.52 $\pm$ 1.41   & 64.06 $\pm$ 0.38    \\
            \midrule
            \rule{0pt}{8pt}
                \tb{\method}
                 &\bf{87.75 $\pm$ 0.68}  & \bf{72.19 $\pm$ 0.60}  & \bf{76.32 $\pm$ 0.28}  & \bf{75.80 $\pm$ 0.19}   \\
            \bottomrule
        \end{tabular}
}
    \vspace{-2.5mm}
\end{table}

==> tables/rebuttal_FT_ZS.tex <==


\begin{table}[H]
    \centering
    \caption{\label{tab:fine_tuning} AUC (in \%) in the detection of dynamic anomaly nodes with fine-tuning variant (SLADE-FT) and zero-shot variant (SLADE-ZS) of SLADE.}
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cccc}
            \toprule
            Method & Wikipedia & Reddit & Bitcoin-alpha & Bitcoin-OTC  \\
            \midrule
            \midrule
                SLADE-FT & 86.06 $\pm$ 0.14   & 60.04 $\pm$ 0.55   & \bf{77.08 $\pm$ 0.17}  & 73.14 $\pm$ 0.61   \\
                SLADE-ZS & 59.15 $\pm$ 0.09   & 53.34 $\pm$ 3.05   & 72.69 $\pm$ 0.02   & 65.00 $\pm$ 0.43    \\
            \midrule
            \rule{0pt}{8pt}
                \tb{\method}
                 &\bf{87.75 $\pm$ 0.68}  & \bf{72.19 $\pm$ 0.60}  & 76.32 $\pm$ 0.28  & \bf{75.80 $\pm$ 0.19}   \\
            \bottomrule
        \end{tabular}
}
    \vspace{-2.5mm}
\end{table}

==> tables/rebuttal_TE.tex <==


\begin{table}[H]
    \centering
    \caption{\label{tab:TE} AUC (in \%) in the detection of dynamic anomaly nodes with a learnable time encoding variant (SLADE-LT) of SLADE and SLADE (SLADE-FT). }
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cccc}
            \toprule
            Method & Wikipedia & Reddit & Bitcoin-alpha & Bitcoin-OTC  \\
            \midrule
            \midrule
                SLADE-LT & 86.78 $\pm$ 0.66   & 65.28 $\pm$ 0.68   & 71.11 $\pm$ 0.83  & 73.98 $\pm$ 0.35   \\
                \tb{\method-FT}
                 &\bf{87.75 $\pm$ 0.68}  & \bf{72.19 $\pm$ 0.60}  & 76.32 $\pm$ 0.28  & \bf{75.80 $\pm$ 0.19}   \\
            \bottomrule
        \end{tabular}
}
    \vspace{-2.5mm}
\end{table}

==> tables/rebuttal_edge_SSL_2.tex <==


\begin{table}[h!]
    \centering
    \caption{\label{tab:Edge_SSL_auc} AUC (in \%) in the detection of dynamic anomaly nodes with baselines based on link prediction self-supervised task.}
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cc}
            \toprule
            Method & Wikipedia & Reddit  \\
            \midrule
            \midrule
                \JODIE (S3)~{\citep{kumar2019predicting}} & 68.88 $\pm$ 1.54   & 58.17 $\pm$ 0.55     \\
                \Dyrep (S3)~{\citep{trivedi2019dyrep}} & 58.78 $\pm$ 4.79   & 59.61 $\pm$ 1.22     \\
                \TGAT (S3)~{\citep{xu2020inductive}}  & 71.40 $\pm$ 2.25   & 59.86 $\pm$ 1.48      \\
                \TGN (S3)~{\citep{tgn_icml_grl2020}}  & 58.05 $\pm$ 3.48   & 56.77 $\pm$ 0.13       \\
            \midrule
            \rule{0pt}{8pt}
                \tb{\method} (S1,S2)
                 &\bf{87.75 $\pm$ 0.68}  & \bf{72.19 $\pm$ 0.60}    \\
            \bottomrule
        \end{tabular}
}
\end{table}

==> tables/rebuttal_hetero.tex <==


\begin{table}[H]
    \centering
    \caption{\label{tab:Hetro} AUC (in \%) in the detection of dynamic anomaly nodes with SLADE and SLADE-Hetero on dynamic bipartite graphs. }
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cc}
            \toprule
            Method & Wikipedia & Reddit   \\
            \midrule
            \midrule
                SLADE & 87.75 $\pm$ 0.68   & 72.19 $\pm$ 0.60     \\
                \tb{\method-Hetero}
                 &\bf{87.96 $\pm$ 0.41}  & \bf{72.65 $\pm$ 0.51}     \\
            \bottomrule
        \end{tabular}
}
    \vspace{-2.5mm}
\end{table}

==> tables/rebuttal_large.tex <==


\begin{table}[H]
    \centering
    \caption{\label{tab:large} AUC (in \%) in the detection of dynamic anomaly nodes with unsupervised baselines in the TGBL-coin dataset.}
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|c}
            \toprule
            Method & TGBL-coin   \\
            \midrule
            \midrule
                \MIDAS~{\citep{bhatia2020midas}} & 56.16 $\pm$ 0.58     \\
                SedanSpot~{\citep{eswaran2018sedanspot}} & 77.14 $\pm$ 0.22  \\
                F-FADE~{\citep{chang2021f}}  & 59.33 $\pm$ 0.00  \\
                Anoedge-l~{\citep{cormode2005improved}}  & 39.11 $\pm$ 2.72  \\
            \midrule
            \rule{0pt}{8pt}
                \tb{\method} 
                 &\bf{83.17 $\pm$ 1.34} \\
            \bottomrule
        \end{tabular}
}
    \vspace{-2.5mm}
\end{table}

==> tables/rebuttal_tolerance.tex <==


\begin{table}[H]
    \centering
    \caption{\label{tab:robust} AUC (in \%) in the detection of dynamic anomaly nodes against additional anomalies in the training set.}
    \setlength{\tabcolsep}{2.5pt}
    %\setlength\aboverulesep{0.6pt}
    \small
    \scalebox{1.0}{
        \def\arraystretch{1.2}
        \begin{tabular}{l|cc}
            \toprule
            Dataset & SLADE & SAD~{\citep{tian2023sad}}   \\
            \midrule
            \midrule
                WIKI+0
                \% & 87.75 $\pm$ 0.68   & 86.15 $\pm$ 0.63     \\
                WIKI+1
                \% & 87.48 $\pm$ 0.56   & 62.64 $\pm$ 13.55     \\
                WIKI+10
                \%  & 87.33 $\pm$ 0.59   & 17.04 $\pm$ 15.77    \\
                WIKI+20
                \%  & 87.05 $\pm$ 3.48   & 33.76 $\pm$ 6.86       \\
            \midrule
                REDDIT+0
                \% & 72.19 $\pm$ 0.60   & 68.45 $\pm$ 1.27     \\
                REDDIT+1
                \% & 72.10 $\pm$ 0.47   & 51.18 $\pm$ 1.28     \\
                REDDIT+10
                \%  & 71.69 $\pm$ 0.92   & 46.64 $\pm$ 0.95    \\
                REDDIT+20
                \%  & 69.97 $\pm$ 4.50   & 47.07 $\pm$ 1.51       \\
            \bottomrule
        \end{tabular}
}
\end{table}

==> tables/selfloop.tex <==
\begin{table}[!t]
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lcc}
            \toprule
            \multirow{2}{*}[-1mm]{Dataset} & \multicolumn{2}{c}{\method} \\
            \cmidrule(lr){2-3}
            & Without Self-loops & With Self-loops (Proposed) \\
            \midrule
            \midrule
            Cora-C      & 80.95 $\pm$ 1.29  & \textbf{81.57 $\pm$ 1.12} \\
            Citeseer    & 71.10 $\pm$ 1.09  & \textbf{72.02 $\pm$ 1.16} \\
            Pubmed      & 84.02 $\pm$ 0.56  & \textbf{84.26 $\pm$ 0.62} \\
            Cora-A      & 79.77 $\pm$ 0.95  & \textbf{82.15 $\pm$ 0.89} \\
            DBLP        & 90.19 $\pm$ 0.12  & \textbf{91.12 $\pm$ 0.11} \\
            Zoo         & \textbf{80.43 $\pm$ 11.3}  & 80.25 $\pm$ 11.2 \\
            20News      & 79.56 $\pm$ 0.24  & \textbf{80.14 $\pm$ 0.19} \\
            Mushroom    & 99.80 $\pm$ 0.14  & \textbf{99.83 $\pm$ 0.13} \\
            NTU2012     & 74.01 $\pm$ 2.54  & \textbf{75.23 $\pm$ 2.45} \\
            ModelNet40  & 93.48 $\pm$ 0.16  & \textbf{97.08 $\pm$ 0.13} \\
            \bottomrule
        \end{tabular}
    }
    \caption{
    Node classification accuracy (\%) of \method when the hypergraphs, which the encoder receives as input, are with and without self-loops.
    Adding self-loops helps to improve the quality of the node representations.
    }
    % Cora-C and Cora-A stand for Cora Co-citation and Cora Co-authorship, respectively.}
    \label{tab:selfloop}
\end{table}


==> tables/training_time_analysis.tex <==
\begin{figure}[!t]
    % \vspace{-1mm}
    \centering
    %\setlength\aboverulesep{0.5pt}
    %\setlength\belowrulesep{0.5pt}
    \centering
    \includegraphics[width=1\linewidth]{figs/appendix_training_time_SLADE.png} 
    \caption{ \label{fig:trianing_time_analysis}
         The left figure shows the increase in the \blue{training time per epoch} of \method with respect to the number of edges in the Reddit dataset. The right figure shows the training time and AUC score (with standard deviations) in the Wikipedia dataset of the competing learning-based methods.
    }
\end{figure}



==> tables/transportation_plot.tex <==
\begin{figure}[H]
    \centering
    \setlength\aboverulesep{0.5pt}
    \setlength\belowrulesep{0.5pt}
    \centering
    \includegraphics[width=1\linewidth]{figs/nyc_taxi_anomaly_score.png} 
    \caption{
    \label{fig:Transportation} Daily average anomaly scores of NYC taxi trips in December 2023. 
    }
\end{figure}

